SCALE: Self-Supervised Constraint-Aware Layout GEneration for Local P&R DRV Fixing at Advanced Nodes

As semiconductor manufacturing advances toward sub-2nm nodes, local place-and-route (P&R) design-rule violation (DRV) fixing is increasingly limited by complex rule interactions, dense multi-layer routing geometries, and foundry-specific constraints. While Large Language Models (LLMs) have recently demonstrated strong capabilities in EDA scripting and documentation, their application to visual layout understanding remains largely unexplored: diagnosing DRC violations from layout imagery demands precise geometric reasoning and foundry-specific rule knowledge absent from general-purpose VLM training. We propose SCALE, a framework with a self-supervised layout-generation stage for local DRV fixing at advanced nodes. Multi-layer layout geometry is serialized into structured text, and a fine-tuned language model learns to reconstruct randomly masked polygons from surrounding BEOL context alone without violation labels. At inference, natural-language rule constraints and high-temperature sampling steer generation toward diverse, violation-prone layout variants validated by an industrial signoff DRC checker, producing DRC-annotated layout--violation pairs used to fine-tune a domain-adapted DRC-VLM. This VLM provides rule-aware geometric guidance for local DRV repair, boosting state-of-the-art agents' solve rates by +12--25% (up to 97%) on 100 real sub-2nm cases spanning enclosure, spacing, width, and color-spacing violations.

==> VLM_ALIGN_DRC_ARXIV/figtexs/CaseStudy_Combined.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.95\textwidth]{figs/CaseStudy_graph_v2.pdf}
    \caption{Examples of DRC fix approaches for VIA spacing (top) and metal tip-to-tip (bottom) rules. (a) Target layouts with the original violations. (b) Baseline agent fixes introduce new violations while try to fix the target DRV. (c) Proposed DRC-VLM analysis with structured root-cause and connectivity-aware actions yielding clean fixes. PRL=Parallel Running Length. \textcolor{blue}{Axis coordinates are scaled for confidentiality.}}
    % \caption{DRC fix examples for VIA spacing (top) and metal tip-to-tip (bottom). (a)~Original violations. (b)~Baseline agent introduces new DRVs. (c)~DRC-VLM-guided fix resolves all violations. PRL=Parallel Running Length. \textcolor{blue}{Axis coordinates are scaled for confidentiality.}}
    \label{fig:case_study}
    \vspace{-10pt}
\end{figure*}


==> VLM_ALIGN_DRC_ARXIV/figtexs/Coverage.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/DataEvalSampleFig.pdf}
    \caption{\textbf{t-SNE Diversity Analysis.} t-SNE projection comparing synthetic datasets against the ground truth (red). Both the trained proposed (autoregressive) and D3PM models achieve high-fidelity, in distribution coverage. In contrast, the heuristic script-based baseline fails to capture the realistic geometric distribution.}
    \Description{t-SNE scatter plots showing overlap of synthetic datasets with ground truth layout distribution.}
    \label{fig:tsne_coverage}
    \vspace{-6pt}
\end{figure}


==> VLM_ALIGN_DRC_ARXIV/figtexs/DR_illustration.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/Figures_for_Complex_rules_illustration.pdf}    \caption{Illustration of VIA layer design rules. (1) \textbf{Basic Rules:} (R1-W) VIA widths are restricted to discrete allowed values $\{W_a, W_b, W_c, \ldots\}$; (R2-Sxx) minimum spacing thresholds are conditioned on the widths of both neighboring VIAs ($W_1$ and $W_2$). (2) \textbf{Group Rules and Group-Conditioned Spacing:} (R3-G) VIAs within a spacing range $[C_1, C_4]$ form groups (e.g., VIA\_GROUP\_2/3) with a maximum count $C_5$ per group; (R2.1-SxxGxH/V) spacing constraints within groups further depend on VIA width, group assignment, orientation (horizontal/vertical), and the parallel run length (PRL) region.}
    \Description{Diagram illustrating VIA design rules including width, spacing, grouping, and group-conditioned spacing constraints.}
    \label{fig:DR}
\end{figure}

==> VLM_ALIGN_DRC_ARXIV/figtexs/Dataset_Aug.tex <==
\begin{figure}[!t]
    % \vspace{-8pt}
    \centering
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/design.pdf}
        \caption{Human design.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/qwen_aug.pdf}
        \caption{Model augmented.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/script_gen.pdf}
        \caption{Script generated. }
    \end{subfigure}

    \caption{Comparison of layout generation methods. Layers are color-coded: \textbf{\textcolor{blue}{Blue} (Mx-1)}, \textbf{\textcolor{green}{Green} (Mx\_A)}, \textbf{\textcolor{cyan}{Cyan} (Mx\_B)}, and \textbf{\textcolor{red}{Red} (VIAx-1)}. (a) Original human-designed layout. (b) Model-augmented layout: the model preserves the original metal routing while generating different via patterns, creating realistic training diversity without altering the routing topology. (c) Script-generated layout: metals and vias are generated using rule-based scripts, resulting in unrealistic metal and via patterns that differ substantially from those found in real designs.}
    % \Description{Three layout crops comparing human-designed, model-augmented, and script-generated VIA placements on metal routing.}
    \label{fig:dataset_aug}
\end{figure}

==> VLM_ALIGN_DRC_ARXIV/figtexs/Framework.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.925\textwidth]{figs/framework_graph_v1.pdf}
    % \caption{\textbf{Proposed Framework.} \textbf{Phase~I (Self-Supervised Layout Generation \& VLM Training):} Multi-layer layout polygons are serialized into a text representation; at training time, random polygon masks teach an autoregressive model the distribution of real design layouts; at inference, high-temperature sampling with various text constraints generates diverse layout variants (e.g., more tip-to-tip metal shapes, additional VIAs). An industrial DRC checker validates generated layouts and a SOTA teacher model produces annotated reasoning traces, forming multi-category supervision for fine-tuning the DRC-VLM.
    % \textbf{Phase~II (Local P\&R DRV Fixing):} Given target local P\&R layouts with DRV reports and design-rule descriptions, the fine-tuned DRC-VLM produces structured expert analysis (root cause, potential fixes, LVS impact). SOTA coding agents (Codex, Claude Code) equipped with DRC/LVS checker tools then execute targeted layout corrections guided by this analysis.}
    %\caption{\textbf{Proposed Framework.} \textbf{Phase~I:} Layouts are serialized into text and used to train an autoregressive model via masked polygon prediction; at inference, text-conditioned sampling generates diverse layouts, which industrial DRC and a teacher model annotate into multi-category supervision for fine-tuning the DRC-VLM. \textbf{Phase~II:} The fine-tuned DRC-VLM analyzes target local P\&R DRVs and provides expert guidance (root cause, fixes, LVS impact) to AI agents that execute the repair.The without predefined actions: it may Move, Size, Add, Remove, etc.}
    \caption{\textbf{Proposed Framework.} \textbf{Phase~I:} Layouts are serialized into text to train an autoregressive model; text-conditioned sampling generates diverse layouts, annotated by industrial DRC and a teacher model for fine-tuning the DRC-VLM. \textbf{Phase~II:} The DRC-VLM guides AI agents to edit the local GDS (boundary polygons may only be extended, not removed) with DRC/LVS checker-in-the-loop feedback.}
    %\Description{Two-phase framework: Phase I shows self-supervised layout generation and VLM training; Phase II shows VLM-guided local P\&R DRV fixing with coding agents.}
    \label{fig:proposed_framework}
    \vspace{-12pt}
\end{figure*}

==> VLM_ALIGN_DRC_ARXIV/figtexs/LayRep.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figs/LayRep_graph_v1.pdf}
%     \caption{Text-formulated layout representation. \textit{Top}: Each polygon is serialized as a coordinate-and-delta token sequence enclosed by \texttt{[Poly]}~\ldots~\texttt{[\textbackslash Poly]} delimiters and grouped under its layer header. \textit{Bottom}: In a real layout crop, metal polygons that extend beyond the crop boundary are marked with \texttt{[BPoly]} (Boundary Polygon) tokens, while fully interior polygons use \texttt{[Poly]}. The LLM receives conditional mixed \texttt{[BPoly]}/\texttt{[Poly]} from different layers as input and generates \texttt{[Poly]} as output, preventing edge-clipping artifacts and enclosure violations from boundary-clipped metal shapes.}
%     \Description{Diagram showing text serialization of layout polygons with coordinate-delta tokens and boundary polygon markers.}
%     \label{fig:layout_representation}
% \end{figure*}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/LayRep_graph_singlecolumn.pdf}
    \caption{Text-formulated layout representation. \textit{Top}: Each polygon is serialized as a coordinate-and-delta token sequence enclosed by \texttt{[Poly]}~\ldots~\texttt{[\textbackslash Poly]} delimiters and grouped under its layer header. \textit{Bottom}: In a real layout crop, metal polygons that extend beyond the crop boundary are marked with \texttt{[BPoly]} (Boundary Polygon) tokens, while fully interior polygons use \texttt{[Poly]}. The LLM receives conditional mixed \texttt{[BPoly]}/\texttt{[Poly]} from different layers as input and generates \texttt{[Poly]} as output, preventing edge-clipping artifacts and enclosure violations from boundary-clipped metal shapes.}
    \Description{Diagram showing text serialization of layout polygons with coordinate-delta tokens and boundary polygon markers.}
    \label{fig:layout_representation}
\end{figure}

==> VLM_ALIGN_DRC_ARXIV/figtexs/Motivation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.425\textwidth]{figs/header_graph_v1.pdf}
    \caption{Off-the-shelf closed-source VLMs hallucinate geometric features (e.g., incorrect VIA count) and lack foundry-specific design rule knowledge, producing inaccurate violation analyses. Our domain-adapted VLM correctly perceives layout geometry and applies precise rule semantics, enabling reliable DRV root cause analysis.}
    \Description{Comparison of VLM outputs on a layout image: a commercial VLM hallucinates geometry while our domain-adapted VLM produces correct violation analysis.}
    \vspace{-10pt}
    \label{fig:motivation}
\end{figure}

==> VLM_ALIGN_DRC_ARXIV/figtexs/SFTPredictionTask.tex <==
\begin{figure}[!t]
    \centering
    % \includegraphics[width=0.5\textwidth]{figs/SFTDataExample_axis.pdf}
    \includegraphics[width=0.48\textwidth]{figs/SFTDataExample_axis.pdf}
    \caption{An example of the VLM detection task used for SFT. 
    Each SFT training pair consists of a layout image, input prompt, and response. \textcolor{blue}{Axis coordinates are scaled for confidentiality.}}
    \label{fig:sftinputexample}
    \vspace{-8pt}
\end{figure}

==> VLM_ALIGN_DRC_ARXIV/tabtex/Ablation1_DataScaling.tex <==
% 50 samples version (archived)
% \begin{table}[!t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Training Samples} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} \\
% \midrule
% 2K            & 20.6\% $\pm$ 2.9\% & 31.7\% $\pm$ 5.3\% & 24.9\% $\pm$ 3.6\% & 6.3\% $\pm$ 1.3\% \\
% 5K            & 26.0\% $\pm$ 2.9\% & 36.9\% $\pm$ 5.7\% & 30.5\% $\pm$ 3.5\% & 8.4\% $\pm$ 1.8\% \\
% 8K            & 24.8\% $\pm$ 2.5\% & \textbf{38.4\%} $\pm$ 3.8\% & 30.2\% $\pm$ 2.7\% & 11.1\% $\pm$ 2.2\% \\
% 16K (full)    & \textbf{44.2\%} $\pm$ 3.5\% & 38.2\% $\pm$ 4.3\% & \textbf{41.0\%} $\pm$ 3.5\% & \textbf{18.3\%} $\pm$ 3.6\% \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Ablation: Effect of training data scale on Mixed (Ours) model (50 samples, $k$=10 trials, avg-trial metrics with 95\% bootstrap confidence intervals). Each model is trained for 1 epoch at GBS=8.}
% \label{tab:ablation_data_scaling}
% \end{table}


%100 samples version
\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Training Samples} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} \\
\midrule
2K            & 21.7\% $\pm$ 2.0\% & 33.7\% $\pm$ 3.5\% & 26.4\% $\pm$ 2.3\% & 7.1\% $\pm$ 1.1\% \\
5K            & 25.4\% $\pm$ 2.3\% & 37.9\% $\pm$ 3.6\% & 30.4\% $\pm$ 2.5\% & 9.0\% $\pm$ 1.7\% \\
10K           & 35.0\% $\pm$ 2.8\% & \textbf{52.5\%} $\pm$ 4.0\% & 42.0\% $\pm$ 3.1\% & 14.9\% $\pm$ 2.6\% \\
16K (full)    & \textbf{46.1\%} $\pm$ 2.8\% & 40.7\% $\pm$ 3.3\% & \textbf{43.3\%} $\pm$ 2.8\% & \textbf{20.7\%} $\pm$ 3.0\% \\
\bottomrule
\end{tabular}%
}
\caption{Ablation: Effect of training data scale on Mixed (Ours) model (100 samples, $k$=10 trials, avg-trial metrics with 95\% bootstrap confidence intervals). Each model is trained for 1 epoch at GBS=8.}
\label{tab:ablation_data_scaling}
\end{table}


==> VLM_ALIGN_DRC_ARXIV/tabtex/Ablation2_DataSource.tex <==
% 50 samples version (archived)
% \begin{table}[h]
% \centering
% \caption{Ablation: Effect of data augmentation source and reasoning traces (50 samples, 13 rules, $k$=10 trials). All models trained for 500 iterations. Training data compositions are detailed in Table~\ref{tab:data_composition}.}
% \label{tab:ablation_data_source}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model Variant} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} \\
% \midrule
% No-reason + ScriptGen aug. & 18.8\% & 37.3\% & 25.0\% &  6.3\% \\
% No-reason + ModelGen aug.  & 37.7\% & 37.9\% & 37.8\% & 17.9\% \\
% Reason + ModelGen aug.     & 44.2\% & 38.2\% & \textbf{41.0\%} & 18.3\% \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[h]
\centering
\caption{Ablation: Effect of data augmentation source and reasoning traces (100 samples, 13 rules, $k$=10 trials). All models trained for 500 iterations. Training data compositions are detailed in Table~\ref{tab:data_composition}.}
\label{tab:ablation_data_source}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Model Variant} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} \\
\midrule
No-reason + ScriptGen aug. & 19.9\% & 39.9\% & 26.6\% &  6.6\% \\
No-reason + ModelGen aug.  & 36.2\% & 36.9\% & 36.5\% & 16.7\% \\
Reason + ModelGen aug.     & \textbf{46.1\%} & 40.7\% & \textbf{43.3\%} & \textbf{20.7\%} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> VLM_ALIGN_DRC_ARXIV/tabtex/DRUnderstanding.tex <==
\begin{table}[h]
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{\textbf{Soft (Rule)}} & \multicolumn{2}{c}{\textbf{Soft (Rule+Loc)}} & \multicolumn{2}{c}{\textbf{Hard (Rule)}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\textbf{Model} & \textbf{P@1} & \textbf{P@3} & \textbf{P@1} & \textbf{P@3} & \textbf{P@1} & \textbf{P@3} \\
\midrule
Qwen 3.5-397B  & 10.4\% & 25.2\% & 7.0\%  & 16.4\% & 0.8\% & 2.4\% \\
GPT-5.2        & 16.9\% & 29.5\% & 15.1\% & 26.1\% & 0.0\% & 0.0\% \\
Gemini 3 Pro   & 20.6\% & 29.0\% & 15.1\% & 22.4\% & 0.0\% & 0.0\% \\
Gemini 2.5 Pro & 27.7\% & 46.2\% & 15.3\% & 26.0\% & 2.8\% & 8.4\% \\
Nemotron-12B   & 33.3\% & 51.2\% & 14.1\% & 20.8\% & 2.4\% & 6.6\% \\
\bottomrule
\end{tabular}%
}
\caption{Model Performance Comparison across Soft and Hard Constraints}
\label{tab:model_performance}
\end{table}

==> VLM_ALIGN_DRC_ARXIV/tabtex/DRVFixTable.tex <==
% \begin{table*}[ht]
% \centering
% \caption{Local DRV fixing Table. Solved Count (SC) and Solve Rate (SR) are reported per DRV rule category and in total. Improvement columns show the absolute SR gain of the DRC-VLM-assisted method over its corresponding baseline.}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|ccccc|c|cccccc}
% \hline
% \multirow{2}{*}{Method}
% & \multicolumn{5}{c|}{DRV Rule Category SC / SR (\%)}
% & {Total}
% & \multicolumn{6}{c}{Impr. (\%)} \\
% \cline{2-6} \cline{8-13}
% & EN & Width & Spacing & Color Spacing & Area
% & SC / SR (\%)
% & EN & Width & Spacing & Color Spacing & Area & Total \\
% \hline
% \textbf{Baselines} & & & & & & & & & & & & \\
% Claude Code
% & 11 (28.2\%) & 26 (96.3\%) & 20 (95.2\%) & 5 (50.0\%) & 1 (33.3\%)
% & 63 (63.0\%)
% & -- & -- & -- & -- & -- & -- \\
% Codex
% & 33 (84.6\%) & 26 (96.3\%) & 18 (85.7\%) & 5 (50.0\%) & \textbf{3 (100.0\%)}
% & 85 (85.0\%)
% & -- & -- & -- & -- & -- & -- \\
% \hline
% \textbf{Proposed} & & & & & & & & & & & & \\
% DRC-VLM + Claude Code
% & 32 (82.1\%) & \textbf{27 (100.0\%)} & \textbf{21 (100.0\%)} & 6 (60.0\%) & 2 (66.7\%)
% & 88 (88.0\%)
% & \textcolor{green!60!black}{+53.8} & \textcolor{green!60!black}{+3.7} & \textcolor{green!60!black}{+4.8} & \textcolor{green!60!black}{+10.0} & \textcolor{green!60!black}{+33.3} & \textcolor{green!60!black}{+25.0} \\
% DRC-VLM + Codex
% & \textbf{39 (100.0\%)} & \textbf{27 (100.0\%)} & \textbf{21 (100.0\%)} & \textbf{7 (70.0\%)} & \textbf{3 (100.0\%)}
% & \textbf{97 (97.0\%)}
% & \textcolor{green!60!black}{+15.4} & \textcolor{green!60!black}{+3.7} & \textcolor{green!60!black}{+14.3} & \textcolor{green!60!black}{+20.0} & +0.0 & \textcolor{green!60!black}{+12.0} \\
% \hline
% \end{tabular}
% }
% \label{tab:drc_pass_rates_improvement}
% \end{table*}


\begin{table*}[ht]
\centering
% \caption{Local DRV fixing results and token cost per case. Baseline agents (Claude Code, Codex) are SOTA coding agents with access to DRC rule descriptions, raw DRC reports, rendered layout images, and DRC/LVS checker tools. Proposed methods augment each agent with expert analysis from DRC-VLM, the strongest model selected from Section~\ref{Sec:VLMSFTExp}. Solved Count (SC) and Solve Rate (SR) are reported per DRV rule category and in total. For proposed methods, absolute SR improvement over the corresponding baseline is shown below each SC/SR value (\textcolor{green!60!black}{green} = higher SR). Average tokens per case are reported in thousands (K); token reduction relative to the corresponding baseline is shown below each token value (\textcolor{green!60!black}{green} = fewer tokens, \textcolor{red}{red} = more tokens). Bold indicates the best value in each column.}
%\caption{Local DRV fixing results and token cost per case. Baseline agents (Claude Code, Codex) are SOTA coding agents with access to DRC rule descriptions, raw DRC reports, rendered layout images, and DRC/LVS checker tools. Proposed methods augment each agent with expert analysis from DRC-VLM, the strongest model selected from Section~\ref{Sec:VLMSFTExp}. Solved Count (SC) and Solve Rate (SR) are reported per DRV rule category and in total. Absolute SR improvement is shown below proposed entries (\textcolor{green!60!black}{green}). Token cost in thousands (K); relative reduction below (\textcolor{green!60!black}{green} = fewer, \textcolor{red}{red} = more). Bold = best.}
\caption{Local DRV fixing results and token cost per case. Baseline agents (Claude Code, Codex) are SOTA coding agents with access to DRC rule descriptions, raw DRC reports, rendered layout images, and DRC/LVS checker tools. Proposed methods augment each agent with expert analysis from DRC-VLM, the strongest model selected from Section~\ref{Sec:VLMSFTExp}. Solved Count (SC) and Solve Rate (SR) are reported per DRV rule category and in total. Absolute SR improvement is shown below proposed entries (\textcolor{green!60!black}{green}). Token cost in thousands (K): Codex reports \texttt{tokens\_used}; Claude Code reports output + cache-creation tokens (excluding cache-read input). Relative reduction below (\textcolor{green!60!black}{green} = fewer, \textcolor{red}{red} = more). Bold = best.}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccc|c|rrrrrr}
\hline
\multirow{2}{*}{Method}
& \multicolumn{5}{c|}{DRV Rule Category SC / SR (\%)}
& {Total}
& \multicolumn{6}{c}{Avg. Tokens / Case (K)} \\
\cline{2-6} \cline{8-13}
& EN & Width & Spacing & Color Spacing & Area
& SC / SR (\%)
& EN & Width & Spacing & Color Spacing & Area & Overall \\
\hline
\textbf{Baselines} & & & & & & & & & & & & \\
Claude Code
& 11 (28.2\%) & 26 (96.3\%) & 20 (95.2\%) & 5 (50.0\%) & 1 (33.3\%)
& 63 (63.0\%)
& 300.8 & 82.0 & 96.2 & 44.4 & 187.7 & 169.7 \\
Codex
& 33 (84.6\%) & 26 (96.3\%) & 18 (85.7\%) & 5 (50.0\%) & \textbf{3 (100.0\%)}
& 85 (85.0\%)
& 96.0 & 82.3 & 92.2 & \textbf{28.4} & \textbf{130.3} & 85.8 \\
\hline
\textbf{Proposed} & & & & & & & & & & & & \\
DRC-VLM + Claude Code
& \begin{tabular}[c]{@{}c@{}}32 (82.1\%)\\{\small \textcolor{green!60!black}{+53.8\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}\textbf{27 (100.0\%)}\\{\small \textcolor{green!60!black}{+3.7\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}\textbf{21 (100.0\%)}\\{\small \textcolor{green!60!black}{+4.8\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}6 (60.0\%)\\{\small \textcolor{green!60!black}{+10.0\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}2 (66.7\%)\\{\small \textcolor{green!60!black}{+33.3\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}88 (88.0\%)\\{\small \textcolor{green!60!black}{+25.0\%}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}214.3\\{\small \textcolor{green!60!black}{(28.7\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}\textbf{74.4}\\{\small \textcolor{green!60!black}{(9.3\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}\textbf{83.0}\\{\small \textcolor{green!60!black}{(13.7\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}\textbf{21.5}\\{\small \textcolor{green!60!black}{(51.5\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}162.4\\{\small \textcolor{green!60!black}{(13.5\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}128.2\\{\small \textcolor{green!60!black}{(24.5\%)}}\end{tabular} \\
DRC-VLM + Codex
& \begin{tabular}[c]{@{}c@{}}\textbf{39 (100.0\%)}\\{\small \textcolor{green!60!black}{+15.4\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}\textbf{27 (100.0\%)}\\{\small \textcolor{green!60!black}{+3.7\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}\textbf{21 (100.0\%)}\\{\small \textcolor{green!60!black}{+14.3\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}\textbf{7 (70.0\%)}\\{\small \textcolor{green!60!black}{+20.0\%}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}\textbf{3 (100.0\%)}\\{\small +0.0\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}\textbf{97 (97.0\%)}\\{\small \textcolor{green!60!black}{+12.0\%}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}\textbf{91.8}\\{\small \textcolor{green!60!black}{(4.6\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}83.5\\{\small \textcolor{red}{(-1.4\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}88.9\\{\small \textcolor{green!60!black}{(3.6\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}29.8\\{\small \textcolor{red}{(-4.9\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}\textbf{130.3}\\{\small (0.0\%)}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}\textbf{83.9}\\{\small \textcolor{green!60!black}{(2.2\%)}}\end{tabular} \\
\hline
\end{tabular}
}
\label{tab:drc_combined}
\end{table*}



==> VLM_ALIGN_DRC_ARXIV/tabtex/DataComposition.tex <==
% \begin{table}[!t]
% \centering
% \caption{Training data composition. Reasoning traces are generated by Gemini-3-Pro; layout descriptions are programmatically extracted from OAS ground-truth layouts. NoR: No Reasoning Trace Violation Data}
% \label{tab:data_composition}
% \small
% \begin{tabular}{lr}
% \toprule
% \textbf{Dataset} & \textbf{Train} \\
% \midrule
% \multicolumn{2}{l}{\textit{Core Components}} \\
% Layout Desc.\ (VIA count \& localization)     & 9,255 \\
% DRC-Reasoning-ModelGen (violation ID w/ reasoning)         & 7,606 \\
% DRC-NoR-ModelGen (model-generated)       & 7,606 \\
% DRC-NoR-ScriptGen (script-generated)     & 6,244 \\
% \midrule
% \multicolumn{2}{l}{\textit{Mixed Training Configurations}} \\
% Mixed-NoR-ScriptGen: Layout Desc. + DRC-NoR-ScriptGen      & 15,499 \\
% Mixed-NoR-ModelGen: Layout Desc. + DRC-NoR-ModelGen       & 16,861 \\
% Mixed (Ours): Layout Desc. + DRC-Reasoning-ModelGen   & 16,861 \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[t]
\caption{Training data composition by generation method and layer type in Section~\ref{Sec:VLMSFTExp}. The DRC analysis task is augmented with reasoning source for the proposed in Table~\ref{tab:combined_metal_via_results}. The description task includes via count, via location, and metal/via bounding box extraction tasks.}
\label{tab:data_composition}
\centering
\small
\begin{tabular}{llrrr}
\hline
\multirow{2}{*}{\textbf{Method}} &
\multirow{2}{*}{\textbf{Layer Type}} &
\multicolumn{1}{c}{\textbf{DRC Analysis}} &
\multicolumn{1}{c}{\textbf{Description}} &
\multirow{2}{*}{\textbf{Total}} \\
& & \multicolumn{1}{c}{\textbf{(w/wo Reasoning)}} &
\multicolumn{1}{c}{\textbf{Task}} & \\
\hline
\multirow{2}{*}{Proposed}
  & VIA   & 7,606 & 9,255  & 16,861 \\
  & Metal & 8,946 & 8,308  & 17,254 \\
\hline
\multirow{2}{*}{Script}
  & VIA   & 6,244 & 9,255  & 15,499 \\
  & Metal & 5,583 & 11,166 & 16,749 \\
\hline
\end{tabular}
\end{table}


==> VLM_ALIGN_DRC_ARXIV/tabtex/MainResults.tex <==
% 50 sample version (archived)
% \begin{table*}[t]
% \centering
% \caption{Model comparison on DRC VLM testing set (50 samples, 13 rules, $k$=10 trials, avg across trials). TP/FP/FN/TN are normalized rule-level rates (\%); overall metrics report 95\% bootstrap confidence intervals. Per-rule F1 columns report macro-average F1 (\%) within each rule category: \textbf{EN}~=~Enclosure (1 rule), \textbf{Grp}~=~Group (1 rule), \textbf{Spc}~=~Spacing (4 rules), \textbf{G-Spc}~=~Group-conditioned Spacing (4 rules), \textbf{W}~=~Width (1 rule). Training data compositions are detailed in Table~\ref{tab:data_composition}. \textsuperscript{$\dagger$}Ablation variants that isolate data source and reasoning contributions.}
% \label{tab:main_results}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lrrrr cccc | ccccc}
% \toprule
% & \multicolumn{4}{c}{\textbf{Confusion Matrix}} & \multicolumn{4}{c|}{\textbf{Overall Metrics}} & \multicolumn{5}{c}{\textbf{Per-Rule Category F1}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-14}
% \textbf{Model} & \textbf{TP}$\uparrow$ & \textbf{FP}$\downarrow$ & \textbf{FN}$\downarrow$ & \textbf{TN}$\uparrow$ & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} & \textbf{EN} & \textbf{Grp} & \textbf{Spc} & \textbf{G-Spc} & \textbf{W} \\
% \midrule
% \multicolumn{14}{l}{\textit{Commercial \& Open-Source Baselines}} \\
% % Qwen 3.5-397B     & 4.0\% & 2.1\% & 35.8\% & 58.1\% &  9.7\% $\pm$ 1.7\% & 20.1\% $\pm$ 3.8\% & 13.0\% $\pm$ 2.3\% &  2.5\% $\pm$ 0.9\% & -- & -- & -- & -- & -- \\
% GPT-5.2           & 6.7\% & 4.8\% & 33.2\% & 55.3\% & 15.4\% $\pm$ 3.6\% & 31.6\% $\pm$ 7.8\% & 20.7\% $\pm$ 4.8\% &  3.1\% $\pm$ 1.3\% &  0 & 41 & 35 &  5 &  0 \\
% Qwen3-VL-8B-Base  & 8.2\% & 6.0\% & 31.6\% & 54.1\% & 19.7\% $\pm$ 3.8\% & 29.7\% $\pm$ 6.0\% & 23.7\% $\pm$ 4.4\% &  2.4\% $\pm$ 1.1\% & 12 & 27 & 33 & 21 &  0 \\
% Gemini 3 Pro      & 8.2\% & 4.4\% & 31.6\% & 55.7\% & 19.9\% $\pm$ 2.7\% & \textbf{66.3}\% $\pm$ 9.1\% & 30.7\% $\pm$ 3.8\% &  8.4\% $\pm$ 2.2\% & \textbf{11} & \textbf{62} & 26 & 28 &  0 \\
% % Gemini 2.5 Pro    & 11.0\% & 10.0\% & 28.9\% & 50.1\% & 27.9\% $\pm$ 3.9\% & 37.7\% $\pm$ 5.6\% & 32.1\% $\pm$ 4.3\% & 11.0\% $\pm$ 2.6\% & -- & -- & -- & -- & -- \\
% % Nemotron-Nano-12B & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multicolumn{14}{l}{\textit{Ours (Qwen3-VL-8B-SFT)}} \\
% \rowcolor{gray!8}
% \quad Mixed-NoR-ScriptGen\textsuperscript{$\dagger$} & 7.6\% & 2.4\% & 32.2\% & 57.8\% & 18.8\% $\pm$ 3.7\% & 37.3\% $\pm$ 7.9\% & 25.0\% $\pm$ 4.8\% &  6.3\% $\pm$ 2.1\% &  0 &  6 & 16 & 33 &  0 \\
% \rowcolor{gray!8}
% \quad Mixed-NoR-ModelGen\textsuperscript{$\dagger$}  & 14.6\% & 9.6\% & 25.2\% & 50.6\% & 37.7\% $\pm$ 4.6\% & 37.9\% $\pm$ 4.4\% & 37.8\% $\pm$ 3.9\% & 17.9\% $\pm$ 4.7\% &  0 & 29 & 30 & 52 &  5 \\
% \rowcolor{gray!15}
% \quad DRC-Reasoning-ModelGen\textsuperscript{$\dagger$} & 9.8\% & 4.6\% & 30.1\% & 55.5\% & 24.6\% $\pm$ 1.9\% & 61.5\% $\pm$ 5.2\% & 35.2\% $\pm$ 2.4\% & 12.3\% $\pm$ 2.0\% &  3 &  5 & 20 & 37 &  0 \\
% \rowcolor{gray!15}
% \quad Mixed (Ours)       & \textbf{17.4\%} & 14.2\% & \textbf{22.4\%} & 45.9\% & \textbf{44.2\%} $\pm$ 3.5\% & 38.2\% $\pm$ 4.3\% & \textbf{41.0\%} $\pm$ 3.5\% & \textbf{18.3\%} $\pm$ 3.6\% &  6 & 33 & \textbf{36} & \textbf{54} & \textbf{23} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


%100 sample version
\begin{table*}[t]
\centering
\caption{Model comparison on DRC VLM testing set (100 samples, 13 rules, $k$=10 trials, avg across trials). TP/FP/FN/TN are normalized rule-level rates (\%); overall metrics report 95\% bootstrap confidence intervals. Per-rule F1 columns report macro-average F1 (\%) within each rule category: \textbf{EN}~=~Enclosure, \textbf{Grp}~=~Group, \textbf{Spc}~=~Spacing, \textbf{G-Spc}~=~Group-conditioned Spacing, \textbf{W}~=~Width. Training data compositions are detailed in Table~\ref{tab:data_composition}. \textsuperscript{$\dagger$}Ablation variants that isolate data source and reasoning contributions.}
\label{tab:main_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrr cccc | ccccc}
\toprule
& \multicolumn{4}{c}{\textbf{Confusion Matrix}} & \multicolumn{4}{c|}{\textbf{Overall Metrics}} & \multicolumn{5}{c}{\textbf{Per-Rule Category F1}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-14}
\textbf{Model} & \textbf{TP}$\uparrow$ & \textbf{FP}$\downarrow$ & \textbf{FN}$\downarrow$ & \textbf{TN}$\uparrow$ & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} & \textbf{EN} & \textbf{Grp} & \textbf{Spc} & \textbf{G-Spc} & \textbf{W} \\
\midrule
\multicolumn{14}{l}{\textit{Commercial \& Open-Source Baselines}} \\
Qwen3-VL-8B-Base  &  9.2\% &  6.1\% & 31.1\% & 53.7\% & 21.5\% $\pm$ 3.0\% & 31.1\% $\pm$ 4.6\% & 25.4\% $\pm$ 3.6\% &  3.7\% $\pm$ 1.1\% &  5\% & 23\% & 33\% & 26\% &  0\% \\
GPT-5.2           & 10.2\% &  6.7\% & 30.0\% & 53.1\% & 23.2\% $\pm$ 3.7\% & 45.7\% $\pm$ 7.8\% & 30.7\% $\pm$ 4.9\% &  4.2\% $\pm$ 1.3\% &  0\% & 48\% & 45\% &  9\% &  0\% \\
Gemini 3 Pro      & 10.7\% &  4.7\% & 29.5\% & 55.1\% & 25.8\% $\pm$ 2.7\% & \textbf{66.9\%} $\pm$ 6.2\% & 37.2\% $\pm$ 3.6\% & 11.0\% $\pm$ 1.7\% &  5\% & \textbf{75\%} & 34\% & 32\% &  0\% \\
\midrule
\multicolumn{14}{l}{\textit{Ours (Qwen3-VL-8B-SFT)}} \\
\rowcolor{gray!8}
\quad Mixed-NoR-ScriptGen\textsuperscript{$\dagger$} &  8.0\% &  2.3\% & 32.3\% & 57.4\% & 19.9\% $\pm$ 2.4\% & 39.9\% $\pm$ 4.9\% & 26.6\% $\pm$ 3.1\% &  6.6\% $\pm$ 1.5\% &  0\% &  7\% & 17\% & 34\% &  0\% \\
\rowcolor{gray!8}
\quad Mixed-NoR-ModelGen\textsuperscript{$\dagger$}  & 14.2\% &  8.9\% & 26.1\% & 50.8\% & 36.2\% $\pm$ 3.1\% & 36.9\% $\pm$ 3.5\% & 36.5\% $\pm$ 3.1\% & 16.7\% $\pm$ 3.2\% &  \textbf{8\%} & 27\% & 28\% & 51\% &  3\% \\
\rowcolor{gray!15}
\quad DRC-Reasoning-ModelGen\textsuperscript{$\dagger$} &  9.6\% &  4.8\% & 30.6\% & 54.9\% & 23.9\% $\pm$ 1.5\% & 59.2\% $\pm$ 3.7\% & 34.1\% $\pm$ 1.9\% & 11.1\% $\pm$ 1.7\% &  1\% &  5\% & 20\% & 36\% &  0\% \\
\rowcolor{gray!15}
\quad Mixed (Ours)       & \textbf{18.4\%} & 14.2\% & \textbf{21.8\%} & 45.6\% & \textbf{46.1\%} $\pm$ 2.8\% & 40.7\% $\pm$ 3.3\% & \textbf{43.3\%} $\pm$ 2.8\% & \textbf{20.7\%} $\pm$ 3.0\% &  2\% & 34\% & \textbf{37\%} & \textbf{57\%} & \textbf{14\%} \\
\bottomrule
\end{tabular}%
}
\end{table*}



==> VLM_ALIGN_DRC_ARXIV/tabtex/PerRuleF1.tex <==
\begin{table}[t]
\centering
\caption{Per-category average F1 (\%) across models (avg across $k$=10 trials, 50 samples). Column abbreviations: \textbf{GPT}~=~GPT-5.2, \textbf{Gem.}~=~Gemini~3~Pro, \textbf{Base}~=~Qwen3-VL-8B-Base, \textbf{S-NoR}~=~Mixed-NoR-ScriptGen\textsuperscript{$\dagger$}, \textbf{M-NoR}~=~Mixed-NoR-ModelGen\textsuperscript{$\dagger$}, \textbf{DRC}~=~DRC-Reasoning-ModelGen\textsuperscript{$\dagger$}, \textbf{Mixed}~=~Mixed (Ours). Daggers denote ablation variants.}
\label{tab:per_rule_f1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc|cccc}
\toprule
& \multicolumn{3}{c|}{\textbf{Baselines}} & \multicolumn{4}{c}{\textbf{Ours}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-8}
\textbf{Category} & \textbf{GPT} & \textbf{Gem.} & \textbf{Base} & \textbf{S-NoR\textsuperscript{$\dagger$}} & \textbf{M-NoR\textsuperscript{$\dagger$}} & \textbf{DRC\textsuperscript{$\dagger$}} & \textbf{Mixed} \\
\midrule
Enclosure (1)         &  0 & \textbf{11} & 12 &  0 &  0 &  3 &  6 \\
Group (1)             & 41 & \textbf{62} & 27 &  6 & 29 &  5 & 33 \\
Spacing (4)           & 35 & 26 & 33 & 16 & 30 & 20 & \textbf{36} \\
Group-cond.\ (4)      &  5 & 28 & 21 & 33 & 52 & 37 & \textbf{54} \\
Width (1)             &  0 &  0 &  0 &  0 &  5 &  0 & \textbf{23} \\
\midrule
\textbf{Macro-avg} (11) & 18 & 26 & 23 & 19 & 33 & 21 & \textbf{38} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> VLM_ALIGN_DRC_ARXIV/tabtex/SFTResultTable.tex <==
% \begin{table*}[t]
% \centering
% \caption{Combined DRC violation detection results across Metal (multi-rule, 100 samples) and VIA (100 samples) layers. Metal uses OAS polygon identity matching; VIA uses centroid distance matching. Overall Comb Score is the arithmetic mean of Metal and VIA Comb F1. All values are pass@$k$ percentages.}
% \label{tab:combined_metal_via_results}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l ccc ccc ccc ccc ccc ccc ccc}
% \toprule
% & \multicolumn{9}{c}{\textbf{Metal Layer}} & \multicolumn{9}{c}{\textbf{VIA Layer}} & \multicolumn{3}{c}{\textbf{Overall}} \\
% \cmidrule(lr){2-10} \cmidrule(lr){11-19} \cmidrule(lr){20-22}
% & \multicolumn{3}{c}{Rule F1 (\%)} & \multicolumn{3}{c}{Loc F1 (\%)} & \multicolumn{3}{c}{Comb F1 (\%)} & \multicolumn{3}{c}{Rule F1 (\%)} & \multicolumn{3}{c}{Loc F1 (\%)} & \multicolumn{3}{c}{Comb F1 (\%)} & \multicolumn{3}{c}{Comb Score (\%)} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}
% \textbf{Model} & @1 & @3 & @5 & @1 & @3 & @5 & @1 & @3 & @5 & @1 & @3 & @5 & @1 & @3 & @5 & @1 & @3 & @5 & @1 & @3 & @5 \\
% \midrule
% \multicolumn{22}{l}{\textit{Commercial \& Open-Source Baselines}} \\
% Gemini-3-Pro & 34.6 & 44.8 & 47.2 & 12.9 & 19.0 & 21.8 & 18.8 & 26.7 & 29.8 & 35.1 & 47.5 & 51.9 & \textbf{15.9} & 24.0 & 27.3 & \textbf{21.9} & 31.9 & 35.8 & 20.4 & 29.3 & 32.8 \\
% GPT-5.2 & 18.2 & 29.2 & 33.4 & 9.7 & 17.5 & 21.1 & 12.7 & 21.9 & 25.9 & 29.7 & 41.3 & 46.9 & 5.1 & 10.4 & 13.8 & 8.7 & 16.6 & 21.3 & 10.7 & 19.3 & 23.6 \\
% Qwen3-Base & 14.6 & 30.7 & 37.3 & 3.5 & 8.9 & 12.9 & 5.7 & 13.8 & 19.2 & 24.1 & 46.5 & 57.4 & 3.9 & 8.7 & 11.8 & 6.7 & 14.7 & 19.5 & 6.2 & 14.3 & 19.4 \\
% \midrule
% \multicolumn{22}{l}{\textit{Qwen3-VL-8B-SFT}} \\
% \rowcolor{gray!8}
%\quad Mixed-NoR-Script\textsuperscript{$\dagger$} & \textbf{49.7} &  \textbf{50.4} & \textbf{50.5} & 1.7 & 3.1 & 3.9 & 3.4 & 5.9 & 7.3 & 24.3 & 46.6 & 57.4 & 7.8 & 17.8 & 24.1 & 11.8 & 25.8 & 34.0 & 7.6 & 15.9 & 20.7 \\
% \rowcolor{gray!8}
% \quad Mixed-NoR-AutoReg\textsuperscript{$\dagger$} & 30.2 & 39.6 & 43.1 & 17.8 & 27.3 & 32.1 & 22.4 & 32.3 & 36.8 & 4.4 & 59.3 & 68.3 & 12.4 & 24.4 & 30.3 & 18.2 & 34.6 & 41.9 & 20.3 & 33.5 & 39.4 \\
% \rowcolor{gray!8}
% \quad DRC-VLM (Proposed) & 47.0 & 49.3 & 50.3 & \textbf{34.3} & \textbf{38.7} & \textbf{40.0} & \textbf{39.6} & \textbf{43.4} & \textbf{44.6} & \textbf{40.6} & \textbf{65.4} & \textbf{72.8} & 12.6 & \textbf{25.1} & \textbf{31.2} & 19.3 & \textbf{36.3} & \textbf{43.7} & \textbf{29.5} & \textbf{39.9} & \textbf{44.2} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

\begin{table}[t]
\centering
% \caption{DRV detection results averaged across Metals and VIAs. Rule F1 and Loc F1 measures rule identification accuracy, and rule-gated violation localization accuracy, respectively. Comb F1 is their harmonic mean. All values are pass@$k$ aggregated over 10 trials. \textsuperscript{$\dagger$}Ablation variants that isolate data source and reasoning contributions.}
\caption{DRV detection results averaged across Metals and VIAs. Rule F1 and Loc F1 measure rule identification and rule-gated localization accuracy; Comb F1 is their harmonic mean. All values are pass@$k$ over 10 trials. \textsuperscript{$\dagger$}Ablations isolating data source and reasoning contributions.}
\label{tab:combined_metal_via_results}
\resizebox{0.48\textwidth}{!}{%
%\scriptsize
\begin{tabular}{l ccc ccc ccc}
\toprule
& \multicolumn{3}{c}{\textbf{Rule F1 (\%)}} & \multicolumn{3}{c}{\textbf{Loc F1 (\%)}} & \multicolumn{3}{c}{\textbf{Comb F1 (\%)}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
\textbf{Model} & @1 & @3 & @5 & @1 & @3 & @5 & @1 & @3 & @5 \\
\midrule
\multicolumn{10}{l}{\textit{Commercial \& Open-Source Baselines}} \\
Gemini-3-Pro & 34.9 & 46.2 & 49.6 & 14.4 & 21.5 & 24.6 & 20.4 & 29.3 & 32.8 \\
GPT-5.2      & 24.0 & 35.3 & 40.2 & 7.4  & 14.0 & 17.5 & 10.7 & 19.3 & 23.6 \\
Qwen3-Base   & 19.4 & 38.6 & 47.4 & 3.7  & 8.8  & 12.4 & 6.2  & 14.3 & 19.4 \\
\midrule
\multicolumn{10}{l}{\textit{Qwen3-VL-8B-SFT}} \\
\rowcolor{gray!8}
\quad Mixed-NoR-Script\textsuperscript{$\dagger$}  & 37.0 & {48.5} & {54.0} & 4.8  & 10.5 & 14.0 & 7.6  & 15.9 & 20.7 \\
\rowcolor{gray!8}
\quad Mixed-NoR-AutoReg\textsuperscript{$\dagger$}  & 17.3 & 49.5 & 55.7 & 15.1 & 25.9 & 31.2 & 20.3 & 33.5 & 39.4 \\
\rowcolor{gray!8}
\quad DRC-VLM (Proposed) & \textbf{43.8} & \textbf{57.4} & \textbf{61.6} & \textbf{23.5} & \textbf{31.9} & \textbf{35.6} & \textbf{29.5} & \textbf{39.9} & \textbf{44.2} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> VLM_ALIGN_DRC_ARXIV/tabtex/TokenCost.tex <==

\begin{table}[!t]
\centering
\caption{Token cost per local DRV fixing case. Average tokens are reported in thousands (K). Percentages under DRC-VLM-assisted values indicate token reduction relative to the corresponding baseline; negative values indicate increased token use.}
\label{tab:token_cost}
\scriptsize
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|rrrrrr}
\toprule
\multirow{2}{*}{\textbf{Method}}
& \multicolumn{6}{c}{\textbf{Avg. Tokens / Case (K)}} \\
\cline{2-7}
& EN & Width & Spacing & Color Spacing & Area & Overall
\\
\midrule
Claude Code
& 2{,}148.4
& 586.1
& 687.2
& 317.5
& 1{,}340.8
& 1{,}212.4 \\
\begin{tabular}[c]{@{}l@{}}DRC-VLM\\+ Claude Code\end{tabular}
& \begin{tabular}[c]{@{}r@{}}1{,}721.7\\{\scriptsize \textcolor{green!60!black}{(19.9\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}591.3\\{\scriptsize \textcolor{red}{(-0.9\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}665.8\\{\scriptsize \textcolor{green!60!black}{(3.1\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}172.7\\{\scriptsize \textcolor{green!60!black}{(45.6\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}1{,}330.4\\{\scriptsize \textcolor{green!60!black}{(0.8\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}1{,}028.1\\{\scriptsize \textcolor{green!60!black}{(15.2\%)}}\end{tabular} \\
\midrule
Codex
& 96.0
& 82.3
& 92.2
& 28.4
& 130.3
& 85.8 \\
\begin{tabular}[c]{@{}l@{}}DRC-VLM\\+ Codex\end{tabular}
& \begin{tabular}[c]{@{}r@{}}91.8\\{\scriptsize \textcolor{green!60!black}{(4.6\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}83.5\\{\scriptsize \textcolor{red}{(-1.4\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}88.9\\{\scriptsize \textcolor{green!60!black}{(3.6\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}29.8\\{\scriptsize \textcolor{red}{(-4.9\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}130.3\\{\scriptsize (0.0\%)}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}83.9\\{\scriptsize \textcolor{green!60!black}{(2.2\%)}}\end{tabular} \\
\bottomrule
\end{tabular}
}
\end{table}

==> VLM_ALIGN_DRC_ARXIV/tabtex/layoutGen.tex <==

% \begin{table}[h]
% \centering
% \caption{Dataset Analysis and Topology Metrics}
% \label{tab:dataset_metrics}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Methods} & \textbf{N} & \textbf{H(M1)} & \textbf{H(V1)} & \textbf{H(M2)} & \textbf{V1 rect\%} & \textbf{V1 unique Topo} & \textbf{VIA Rules Triggered} \\
% \midrule
% Training Samples (1k)  & 1,000 & 1.84 & 1.63 & 1.63 & 100\% & 24  & -- \\
% Design Layout Samples(15k) & 4,000 & 2.19 & 1.67 & 2.44 & 100\% & 31  & -- \\
% % D3PM Raw              & 4,000 & 2.19 & 3.52 & 2.44 & 92\%  & 136 & -- \\
% D3PM     & 4,000 & 2.19 & 2.99 & 2.44 & 100\% & 60  & 18 \\
% Qwen-SFT              & 4,000 & 2.46 & 3.36 & 2.66 & 100\% & 88  & 22 \\
% Agent+Script      & 4,000 & 0.69 & 3.04 & 3.77 & 100\% & 48  & 10 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

% original big table
% \begin{table*}[t]
% \centering
% \caption{Pattern diversity comparison across generation methods. $H$ is the Shannon entropy of the joint complexity distribution $P(c_x, c_y)$. Higher $H$ indicates more diverse layout patterns. DRC columns report design rule violation metrics for VIA and Metal layers separately.}
% \label{tab:pattern_diversity}
% \scriptsize
% \begin{tabular}{lccc|ccccc|ccccc}
% \toprule
% & & & & \multicolumn{5}{c|}{\textbf{VIA DRC}} & \multicolumn{5}{c}{\textbf{Metal DRC}} \\
%\cmidrule(lr){5-9} \cmidrule(lr){10-14}
%\textbf{Method} & \textbf{N} & \textbf{H} $\uparrow$ & \textbf{Unique} & \textbf{W} & \textbf{Spc} & \textbf{G-Spc} & \textbf{EN} & \textbf{Grp}  & \textbf{W/A} & \textbf{Spc} & \textbf{EN} & \textbf{R} & \textbf{CS} \\
%\midrule
%Training Data                  & 2.0K & 2.93 &  93  & -- & -- & -- & -- & -- & -- & -- & -- & -- & \\
%D3PM Conditional               & 14.9K & 4.61 & 236  & 1 & 5 & 3 & 7 & 2 & 5 & 4 & 2 & 1 & 1 \\
%Script                         & 28.0K & 3.94 & 133  & 2 & 3 & 2 & 1 & 2 & 7 & 2 & 2 & 1 & 0 \\
%Proposed                       & 17.7K & 5.07 & 289  & 1 & 13 & 7 & 6 & 3 & 13 & 4 & 4 & 10 & 3 \\
%\bottomrule
%\end{tabular}%
%\end{table*}  


% \begin{table}[t]
%\centering
%\caption{Pattern diversity comparison across generation methods. $H$ is the Shannon entropy of the joint complexity distribution $P(c_x, c_y)$. Higher $H$ indicates more diverse layout patterns. DRC columns report design rule violation metrics for VIA and Metal layers separately. DRC columns report unique validated triggered rules by category (VIA / Metal). Abbreviations: W = Width, W+A = Width + Area, Spc = Spacing, G-Spc = Group-conditioned Spacing, EN = Enclosure, Grp = Group, R = Routing, CS = Colored Spacing.}
%\label{tab:dataset_metrics}
%\scriptsize
%\setlength{\tabcolsep}{2pt}
%\begin{tabular}{lccc|cccccc}
%\toprule
%\textbf{Method} & \textbf{N} & \textbf{H} $\uparrow$ & \textbf{Unique Top.} & \multicolumn{6}{c}{\textbf{Validated VIA / Metal DRV Type}}  \\
%\cmidrule(lr){5-10} 
%& &  &  & \textbf{W / W+A} & \textbf{Spc} &  \textbf{EN} & \textbf{G-Spc / R}  & \textbf{Grp / CS} & \textbf{Total} \\
%\midrule
%Training Data                  & 1.0K & 2.93 &  93  & -- & -- & -- & -- & -- & -- \\
%D3PM                           & 14.9K & 4.61 & 236  & 1 / 5 & 5 / 4 & 7 / 2 & 3 / 1  & 2 / 1 & 18 / 13 \\
%Script                         & 28.0K & 3.94 & 133  & 2 / 7 & 3 / 2 & 1 / 2 & 2 / 1  & 2 / 0 & 10 / 12 \\
%Proposed                       & 17.7K & 5.07 & 289  & 1 / 13 & 13 / 4  & 6 / 4 & 7 / 10  & 3 / 3 & 29 / 34 \\
%\bottomrule
%\end{tabular}%
%\end{table}

\begin{table}[t]
\centering
\caption{Pattern diversity comparison across generation methods. $H$ is the Shannon entropy of the joint complexity distribution $P(c_x, c_y)$. Higher $H$ indicates more diverse layout patterns. DRC columns report design rule violation metrics for VIA and Metal layers separately. DRC columns report unique validated triggered rules by category (VIA / Metal). Abbreviations: W = Width, W+A = Width + Area, Spc = Spacing, G-Spc = Group-conditioned Spacing, EN = Enclosure, Grp = Group, R = Routing, CS = Colored Spacing.}
\label{tab:dataset_metrics}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcc|cccccc}
\toprule
\textbf{Method} & \textbf{H} $\uparrow$ & \textbf{Unique Top.} & \multicolumn{6}{c}{\textbf{Validated VIA / Metal DRV Type}}  \\
\cmidrule(lr){4-9} 
& &  & \textbf{W / W+A} & \textbf{Spc} &  \textbf{EN} & \textbf{G-Spc / R}  & \textbf{Grp / CS} & \textbf{Total} \\
\midrule
Training Data                  & 2.93 &  93  & -- & -- & -- & -- & -- & -- \\
D3PM                           & 4.61 & 236  & 1 / 5 & 5 / 4 & 7 / 2 & 3 / 1  & 2 / 1 & 18 / 13 \\
Script                         & 3.94 & 133  & 2 / 7 & 3 / 2 & 1 / 2 & 2 / 1  & 2 / 0 & 10 / 12 \\
Proposed                       & 5.07 & 289  & 1 / 13 & 13 / 4  & 6 / 4 & 7 / 10  & 3 / 3 & 29 / 34 \\
\bottomrule
\end{tabular}%
\end{table}

==> VLM_ALIGN_DRC_ARXIV/tex/0_abstract.tex <==

\begin{abstract}
% As semiconductor manufacturing advances toward sub-2nm nodes, the complexity of design rules has escalated due to stringent constraints from EUV lithography and 3D transistor architectures, making DRC violation understanding a critical bottleneck in achieving design closure.
% While Large Language Models (LLMs) have recently demonstrated strong capabilities in EDA scripting and documentation, their application to \emph{visual} layout understanding remains largely unexplored: diagnosing DRC violations from layout imagery demands precise geometric reasoning and foundry-specific rule knowledge absent from general-purpose VLM training.
% In this work, we propose a three-phase framework to align Vision-Language Models (VLMs) with VLSI geometry through scalable synthetic data generation, reasoning-augmented data curation, and domain-adapted fine-tuning.
% In this work, we propose \emph{GeoDRC-VLM}, a rule-aware synthetic layout generation framework for adapting vision-language models (VLMs) to advanced-node geometric design-rule reasoning. 
% Our autoregressive layout generation pipeline integrate text constraints with layout generation procedures to generate diverse, signoff-verified layout--violation samples. 
% The layout generation pipeline is which are used to supervise geometry grounding, rule reasoning, and layout description for a domain-adapted Qwen3-VL-8B model.
% We introduce an autoregressive layout augmentation pipeline in which a fine-tuned LLM generates diverse, signoff-verified layout--violation pairs under advanced-node DRC constraints.
% We then fine-tune an open-source VLM (Qwen3-VL-8B) with multi-category supervision, spanning VIA and metal spatial localization together with step-by-step reasoning traces, to jointly learn geometric grounding and rule-based diagnostic reasoning.
% We demonstrate that our domain-adapted 8B model outperforms state-of-the-art baselines by 9.35\% on average in rule identification, with ablations confirming that data quality and reasoning supervision are complementary on an industrial sub-2nm process design kit (PDK).
% Experimental results show that our domain-adapted 8B model outperforming state-of-the-art baselines by 14.6\% on rule identification on average, with ablations confirming that data quality and reasoning supervision are complementary.
% All experiments are validated on an industrial sub-2nm process design kit (PDK).
As semiconductor manufacturing advances toward sub-2nm nodes, local place-and-route (P\&R) design-rule violation (DRV) fixing is increasingly limited by complex rule interactions, dense multi-layer routing geometries, and foundry-specific constraints. While Large Language Models (LLMs) have recently demonstrated strong capabilities in EDA scripting and documentation, their application to \emph{visual} layout understanding remains largely unexplored: diagnosing DRC violations from layout imagery demands precise geometric reasoning and foundry-specific rule knowledge absent from general-purpose VLM training.

% We propose \emph{SCALE}, a self-supervised synthetic layout generation framework for local DRV fixing at advanced nodes. Multi-layer layout geometry is serialized into structured text, and a fine-tuned language model learns to predict randomly masked polygons conditioned on surrounding BEOL context and natural-language rule constraints, requiring no violation labels. At inference, controllable sampling and text prompts generate diverse, realistic layout variants, which are validated and annotated by industrial signoff DRC to produce layout--violation pairs for VLM training.
% Using the generated data, we fine-tune an open-source VLM to provide rule-aware geometric guidance for local DRV repair. \emph{SCALE} improves fixing pass rates on local P\&R layout regions extracted from real designs, spanning spacing, intricate conditional enclosure, patterning, and multi-layer metal/via spacing violations, boosting SOTA agents' solve rates by +12--25\% (up to 97\%) on 100 real sub-2\,nm cases. These results demonstrate that self-supervised, constraint-aware synthetic layout generation can translate advanced-node geometric reasoning into practical local P\&R DRV fixing across diverse, interaction-heavy rule scenarios.

We propose \emph{SCALE}, a framework with a self-supervised layout-generation stage for local DRV fixing at advanced nodes. Multi-layer layout geometry is serialized into structured text, and a fine-tuned language model learns to reconstruct randomly masked polygons from surrounding BEOL context alone without violation labels. At inference, natural-language rule constraints and high-temperature sampling steer generation toward diverse, violation-prone layout variants validated by an industrial signoff DRC checker, producing DRC-annotated layout--violation pairs used to fine-tune a domain-adapted DRC-VLM.
This VLM provides rule-aware geometric guidance for local DRV repair, boosting state-of-the-art agents' solve rates by +12--25\% (up to 97\%) on 100 real sub-2\,nm cases spanning enclosure, spacing, width, and color-spacing violations.

%Using the generated data, we fine-tune an open-source VLM to provide rule-aware geometric guidance for local DRV repair. SCALE improves fixing pass rates on local P\&R layout regions extracted from real designs, spanning spacing, intricate conditional enclosure, patterning, and multi-layer metal/via spacing violations, increasing state-of-the-art agents from 74.0\% to 92.5\% on average. These results demonstrate that self-supervised, constraint-aware synthetic layout generation can translate advanced-node geometric reasoning into practical local P\&R DRV fixing across diverse, interaction-heavy rule scenarios.
\end{abstract}

==> VLM_ALIGN_DRC_ARXIV/tex/1_introduction.tex <==

\vspace{-6pt}
\section{INTRODUCTION}
% \vspace{-4pt}

%Design Rule Checking (DRC) and Violation (DRV) correction have emerged as critical bottlenecks in achieving design closure at advanced process nodes.
%At sub-2\,nm nodes, EUV lithography, 3D transistor architectures, and Design-Technology Co-optimization (DTCO) have introduced hundreds of conditional, \emph{topology-dependent} constraints, e.g., conditional enclosure, group- and color-dependent spacing, and discrete width quantization, whose legality depends jointly on neighboring wire widths, multi-layer enclosure, and double-patterning color assignment, far beyond the fixed-width/spacing checks of earlier nodes.
%Commercial signoff checkers~\cite{Calibre} only \emph{detect} such violations, leaving a human engineer to manually interpret and hand-fix each one, an unscalable process at SoC scale.
%In-design DRC and detail-routing/ECO engines~\cite{Innovus,ICC2} fix violations automatically only by encoding each rule as a hand-tuned geometric constraint or correction template~\cite{DRC+}; as rules grow increasingly conditional, this rule-by-rule engineering effort cannot keep pace, leaving many complex rules uncovered and local repairs prone to cascading new violations onto adjacent layers under double-patterning and multi-layer stacking.
%A more flexible, automated approach to local DRV fixing is therefore needed, one that neither signoff checkers nor template-based correction currently provide.

Design Rule Checking (DRC) and Violation (DRV) correction have emerged as critical bottlenecks in achieving design closure at advanced process nodes.
At sub-2\,nm nodes, EUV lithography and Design-Technology Co-optimization (DTCO) have introduced hundreds of conditional, topology-dependent constraints (e.g., conditional enclosure, color-dependent spacing, discrete width quantization) whose legality depends jointly on neighboring geometries, multi-layer enclosure, and double-patterning color assignment.
Commercial signoff checkers~\cite{Calibre} only \emph{detect} such violations, leaving engineers to manually interpret and fix each one.
In-design DRC and detail-routing engines~\cite{Innovus,ICC2} fix violations automatically but rely on hand-tuned geometric templates~\cite{DRC+}; as rules grow increasingly conditional, this rule-by-rule approach cannot keep pace, leaving complex rules uncovered and local repairs prone to cascading new violations.
A more flexible, automated approach to local Place-and-Route (P\&R) DRV fixing is therefore needed.



\input{figtexs/Motivation}
% Para 2: WHAT'S BEEN TRIED — LLMs offer flexible, language-specified fixing, but need visual grounding + training data
%Large Language Models (LLMs) offer a promising alternative to template-based correction: since design rules are ultimately textual, an LLM agent can interpret a rule constraint in natural language and propose a targeted fix without hard-coding it into a routing engine.
%Prior EDA work applies LLMs to \emph{text-centric} tasks: documentation retrieval~\cite{ORAssistant}, DRC checker code generation~\cite{DRCCoder,kim2026rule2drc}, and RAG/CoT script automation~\cite{DocumentQA_ICCAD}. These agents synthesize checker code from rule text, whereas DRV fixing additionally requires visually grounding a rule in the local layout, a step largely unexplored for vision-language models (VLMs).
%As Fig.~\ref{fig:motivation} shows, off-the-shelf VLMs fail at this grounding: they hallucinate geometric features and lack the domain knowledge to map visual patterns onto rule semantics, so an agent relying on such analysis inherits these errors and misfixes or reintroduces violations.
%Textual rule descriptions alone cannot supply this grounding, and no structured layout--violation dataset exists to teach it, making fine-tuning-based domain adaptation impractical.

Large Language Models (LLMs) offer a promising alternative: since design rules are textual, an LLM agent can interpret a rule constraint and propose a targeted fix without hard-coding it into a routing engine.
Prior EDA work applies LLMs to text-centric tasks such as documentation retrieval~\cite{ORAssistant}, DRC checker code generation~\cite{DRCCoder,kim2026rule2drc}, and script automation~\cite{DocumentQA_ICCAD}, but DRV fixing additionally requires visually grounding a rule in the local layout, a capability largely unexplored for vision-language models (VLMs).
As Fig.~\ref{fig:motivation} shows, off-the-shelf VLMs fail at this grounding: they hallucinate geometric features and lack the domain knowledge to map visual patterns onto rule semantics, causing agents that rely on them to misfix or reintroduce violations.
No structured layout--violation dataset exists to teach this grounding, making fine-tuning-based domain adaptation impractical.


% Para 3: THE GAP — data scarcity + domain gap (why this is uniquely hard)
% Constructing such training data faces two barriers.
%First, \emph{data scarcity}: production layouts are predominantly DRC-clean, real violations skew toward a narrow rule subset, and layouts synthesized by agentic methods from rule descriptions alone fail to reproduce real DRVs, leaving too few usable layout--violation examples to train on.
%Second, a \emph{domain gap}: complex, conditional design rules are confidential to foundries, so VLMs pretrained on public, natural-world images have never seen this geometry, and their spatial reasoning, tuned for everyday photos, does not generalize to nanometer-scale VLSI layouts.
%Overcoming both, generating high-quality, real-layout-scenario DRVs at scale, is the core challenge this work addresses.
Constructing such training data faces two barriers.
First, \emph{data scarcity}: production layouts are predominantly DRC-clean, real violations skew toward a narrow rule subset, and agentic synthesis from rule descriptions alone fails to reproduce realistic DRVs.
Second, a \emph{domain gap}: conditional design rules are foundry-confidential, so VLMs pretrained on public, natural-world images have never encountered nanometer-scale VLSI geometry and cannot generalize their spatial reasoning to it.
Overcoming both barriers is the core challenge this work addresses.

% Two barriers make this problem uniquely challenging.
%First, \emph{severe data scarcity}: production layouts are predominantly DRC-clean, the few violations that occur are biased toward a narrow subset of rules, and privacy constraints on foundry PDKs preclude public dataset construction.
%Second, a \emph{fundamental domain gap}: VLSI layout semantics are governed by nanometer-precision geometric rules rather than natural-world physics, rendering the spatial priors of general-purpose VLMs ineffective.
%Bridging both gaps simultaneously, generating diverse rule-annotated training data \emph{and} adapting a VLM to VLSI geometry, is the core challenge this work addresses.
\input{figtexs/Framework}
% Para 4: OUR INSIGHT + APPROACH + RESULTS
% In this work, we serialize multi-layer layout geometry into text and train a language model with a \emph{self-supervised} masked-prediction objective: the model reconstructs masked polygons conditioned on surrounding BEOL context and an optional natural-language rule constraint, requiring no violation labels at training time.
% This decouples generation from labeling: at inference, sampling under different text prompts and temperatures yields diverse, realistic layout variants targeting specific rule families, which industrial signoff DRC verifies and annotates into layout--violation pairs at scale.
% Because target rules are specified in flexible text rather than hard-coded into a routing/ECO engine, the same generator retargets to new, complex conditional rules by prompt alone, without additional rule engineering.
% We then fine-tune an open-source VLM~\cite{Qwen3VL} on the resulting corpus with layout perception, violation, and reasoning-trace supervision, yielding a rule-aware, domain-adapted DRC-VLM that guides a state-of-the-art (SOTA) coding agent to fix local P\&R DRVs that neither commercial checkers nor unguided agents can resolve.
% The main contributions of this work are as follows:
% In this work, we address both barriers with a self-supervised pipeline that generates diverse layout--violation pairs at scale from real designs, without manually creating or labeling DRV layouts.
%Because target rule families are specified in flexible text rather than hard-coded as routing-engine code, the same model retargets to new, complex conditional rules by prompt alone, with no nontrivial labeling effort.
%We then fine-tune an open-source VLM~\cite{Qwen3VL} on the resulting corpus, yielding a rule-aware, domain-adapted DRC-VLM that guides a state-of-the-art~(SOTA) coding agent to fix local place-and-route (P\&R) DRVs that neither commercial checkers nor unguided agents can resolve.
% The main contributions of this work are as follows:


%In this work, we address both barriers with a self-supervised pipeline that generates diverse layout--violation pairs at scale from real designs, without hard-coding target rules into a routing/ECO engine or creating the DRV layouts manually.
%We then fine-tune an open-source VLM~\cite{Qwen3VL} on the resulting corpus, yielding a rule-aware, domain-adapted DRC-VLM that guides a state-of-the-art~(SOTA) agent to fix local P\&R DRVs that neither commercial checkers nor unguided agents can resolve.
%The main contributions of this work are as follows:

% In this work, we address both barriers with a self-supervised pipeline that generates diverse layout--violation pairs at scale from real designs, without hard-coding target rules into a routing/Engineering Change Order (ECO) engine or creating the DRV layouts manually.
Here, we address both barriers with a pipeline whose self-supervised generation stage produces diverse layout--violation pairs at scale from real designs, without hard-coding target rules into a routing/Engineering Change Order (ECO) engine or creating the DRV layouts manually.
We then fine-tune an open-source VLM~\cite{Qwen3VL} on the resulting corpus, yielding a rule-aware, domain-adapted DRC-VLM that guides a state-of-the-art~(SOTA) coding agent to fix local P\&R DRVs more efficiently and effectively than unguided agents alone, addressing violations that commercial signoff checkers can only detect but not repair.
The main contributions of this work are as follows:
% \vspace{-4pt}

\iffalse
\begin{itemize}[nosep,topsep=2pt,leftmargin=*]

   % lead with the end-to-end data pipeline, then how that data targets DRV fixing scenarios, then the supporting studies, then the headline fixing result.
    \item \textbf{End-to-End Generative VLM-DRC Framework.} 
    We introduce \emph{SCALE}, a comprehensive framework that bridges the layout-to-violation domain gap. It unifies a self-supervised text-formulated polygon generator and a domain-adapted vision-language model (DRC-VLM) optimized specifically for multi-category geometric reasoning and advanced-node design rule interactions.\textcolor{red}{Add training data curation with description task and DRV analysis} 
    We curate multi-category supervision, including layout perception, violation labels, and reasoning traces, to teach the VLM rule-aware geometry understanding beyond simple object localization. This supervision helps the model identify violation-causing regions and supports diverse, scenario-dependent DRV repair cases that are difficult to enumerate manually.
    % \item \textbf{End-to-end multi-modal data generation pipeline from real layouts.}
    % We propose \emph{SCALE}, which fine-tunes a language model to reconstruct masked polygons in a text-formulated layout representation, conditioned on real BEOL context and optional natural-language rule constraints, requiring no violation labels for training. At inference, text-conditioned sampling flexibly targets complex conditional rules, while industrial signoff DRC checker verifies the generated layouts and produces scalable multi-modal (image, GDS, text) layout--violation pairs.

    \item \textbf{Self-Supervised, Rule-Conditioned Layout-Violation Synthesis.} 
    As the data foundation of \emph{SCALE}, we develop an LLM-based generation pipeline that, trained on real design layouts, reconstructs masked polygons conditioned on the surrounding BEOL context and natural-language constraints. The generated variants are then filtered through an industrial signoff DRC checker, yielding layout--violation pairs at scale without any pre-labeled training data.


    %\item \textbf{Comprehensive data generation and ablation studies.}
    %We comprehensively evaluate the data generation pipeline against a discrete-diffusion~\cite{PatternPaint} baseline and an agentic script-based generator. Our pipeline generates the most diverse layout topologies, triggers the broadest local P\&R DRC rule coverage, and better matches real-layout distributions, while ablations show that data quality and scale consistently improve downstream DRV detection.

    \item \textbf{Empirical Validation and SOTA Local P\&R DRV Fixing at Sub-2\,nm.}
    %We apply the fine-tuned DRC-VLM on 100 real local P\&R fixing scenarios from a sub-2\,nm design, where its expert guidance raises SOTA coding agents' average solve rate from 74.0\% to 92.5\% across enclosure, width, spacing, color-spacing, and area violations.
    We conduct holistic studies on our data generation against discrete-diffusion and agentic baselines, demonstrating superior topology diversity and rule coverage. Crucially, we deploy the complete \emph{SCALE} framework on 100 real sub-2\,nm local P\&R fixing scenarios, where its expert visual guidance elevates the DRV solve rate of state-of-the-art coding agents from 74.0\% to 92.5\% across enclosure, width, spacing, color-spacing, and area violations.

     \item \textbf{End-to-End Generative VLM-DRC Framework.} 
    We introduce \emph{SCALE}, a comprehensive framework that bridges the layout-to-violation domain gap. It unifies a self-supervised text-formulated polygon generator and a domain-adapted vision-language model (DRC-VLM) optimized specifically for multi-category geometric reasoning and advanced-node local P\&R design rule interactions.

    \item \textbf{Self-Supervised Synthesis and Multi-Task Data Curation.} 
    We develop an LLM-based pipeline that reconstructs masked polygons conditioned on BEOL context and natural-language constraints, verified by an industrial signoff checker to yield labeled pairs at scale. On top of this corpus, we curate multi-category instruction-tuning data---layout descriptions, violation labels, and step-by-step DRV reasoning traces---enabling the VLM to pinpoint complex, scenario-dependent violations beyond simple object localization.
    % As the data foundation of \emph{SCALE}, we develop an LLM-based generation pipeline that, trained on real design layouts, reconstructs masked polygons conditioned on the surrounding BEOL context and natural-language constraints, which are then verified via an industrial signoff DRC checker to yield unlabeled pairs at scale. On top of this corpus, we curate multi-category instruction-tuning data—including dedicated layout description tasks, precise violation labels, and step-by-step DRV analysis reasoning traces—to teach the VLM rule-aware geometry understanding beyond simple object localization, enabling it to pinpoint complex, scenario-dependent violation regions.

    \item \textbf{Empirical Validation and SOTA Local P\&R DRV Fixing at Sub-2\,nm.} 
    %We conduct holistic studies on our data generation against discrete-diffusion and agentic baselines, demonstrating superior topology diversity and rule coverage. Crucially, we deploy the complete \emph{SCALE} framework on 100 real sub-2\,nm local P\&R fixing scenarios, where its expert visual guidance elevates the DRV solve rate of state-of-the-art coding agents from 74.0\% to 92.5\% across enclosure, width, spacing, color-spacing, and area violations.
    We conduct holistic studies on our data generation against discrete-diffusion and agentic baselines, demonstrating superior topology diversity and rule coverage. On 100 real sub-2\,nm local P\&R fixing scenarios, DRC-VLM's expert visual guidance elevates the DRV solve rate of SOTA agents from 74.0\% to 92.5\% across enclosure, width, spacing, color-spacing, and area violations.
\end{itemize}
\fi

\begin{itemize}[nosep,topsep=2pt,leftmargin=*]

    \item \textbf{Self-Supervised, Rule-Conditioned DRV Data Generation from Real Layouts.}
%    We introduce \emph{SCALE} and develop an LLM-based generation pipeline that reconstructs masked polygons conditioned on BEOL context and natural-language rule constraints, requiring no violation labels for training. An industrial signoff checker verifies the generated layouts, yielding diverse layout--violation pairs at scale from real designs.
    We introduce \emph{SCALE} and develop an LLM-based generation pipeline that reconstructs masked polygons from BEOL context alone without violation labels. At inference, natural-language constraints steer sampling toward violation-prone configurations, and an industrial signoff checker verifies the outputs, yielding diverse layout--violation pairs at scale from real designs.


    \item \textbf{Constraint-Aware Data Curation and Domain-Adapted DRV Fixing.}
    On top of the generated corpus, we curate multi-category supervision (layout descriptions, violation labels, and step-by-step reasoning traces) to fine-tune a domain-adapted DRC-VLM. This model provides dynamic, rule-conditioned guidance to SOTA coding agents for local P\&R DRV repair.

    \item \textbf{Empirical Validation and SOTA Local P\&R DRV Fixing at Sub-2\,nm.} % We conduct holistic studies on our data generation against discrete-diffusion and agentic baselines, demonstrating superior topology diversity and rule coverage. On 100 real sub-2\,nm local P\&R fixing scenarios, DRC-VLM guidance elevates the DRV solve rate of SOTA coding agents from 74.0\% to 92.5\% across enclosure, width, spacing, color-spacing, and area violations.
    We conduct holistic studies on our data generation against discrete-diffusion and agentic baselines, demonstrating superior topology diversity and rule coverage. On 100 real sub-2\,nm local P\&R fixing scenarios, DRC-VLM guidance boosts SOTA agents' solve rates by +12--25\% (up to 97\%) across enclosure, width, spacing, color-spacing, and area violations.



\end{itemize}



==> VLM_ALIGN_DRC_ARXIV/tex/2_relatedwork.tex <==
% \vspace{-6pt}
% \section{Preliminaries}
% \vspace{-4pt}
% \subsection{Motivating Example}

% \input{figtexs/DR_illustration}
% Already mentioned in introduction and experiements; save space
% As illustrated in Fig.~\ref{fig:DR}, design constraints at advanced nodes have evolved from simple static checks (e.g., fixed width/spacing) to conditional rules where legality depends on the surrounding topology. At the basic level, VIA widths are restricted to discrete allowed values (Fig.~\ref{fig:DR}, R1-W) and minimum spacing thresholds depend on the widths of both neighboring VIAs (Fig.~\ref{fig:DR}, R2-Sxx). Beyond these pairwise constraints, VIAs within certain spacing ranges form groups (Fig.~\ref{fig:DR}, R3-G) with maximum count limits, and group-conditioned spacing rules (Fig.~\ref{fig:DR}, R2.1) introduce further dependencies on VIA width, group assignment, orientation, and parallel run length (PRL). 
% In practice, via legality depends not only on the intersection between lower and upper metal layers, but also on rich local context, including double-patterning constraints, enclosure and spacing rules, multi-layer stacking requirements, and dummy-fill interactions. 
% This complexity makes correctly identifying \emph{which} rules are violated, \emph{where} violations occur, and \emph{why} they arise a task that requires deep geometric reasoning over multi-layer layout topology and remains largely manual and expert-dependent.
%\vspace{-6pt}
%\section{Related Work}

%\input{figtexs/Framework}
% \noindent\textbf{LLMs and VLMs for EDA.}
%LLMs have been widely adopted for text- and code-centric EDA tasks: documentation QA~\cite{ORAssistant, DocumentQA_ICCAD}, chip design assistance~\cite{liu2023chipnemo}, RTL generation~\cite{ho2025verilogcoder, wan2025schemacoder}, formal verification~\cite{wan2026fvrulelearner}, and general scientific reasoning~\cite{ho2026polymath}.
%For design rule understanding, DRC-Coder~\cite{DRCCoder} and Rule2DRC~\cite{kim2026rule2drc} combine VLMs and LLMs to automatically generate DRC checker code from rule descriptions, achieving strong accuracy on synthesizing rule-implementing programs. These works address a fundamentally different problem from ours: they generate \emph{checker code} before any violation occurs, whereas our work starts \emph{after} a violation has been flagged, using a VLM to visually ground it in the layout, diagnose its root cause, and guide an agent to repair it.
%In a complementary data-centric direction, CraftRTL~\cite{CraftRTL} and ScaleRTL~\cite{ScaleRTL} show that synthetic data curation and reasoning-trace supervision can substantially improve LLM performance under data scarcity for RTL generation. We share this data-centric philosophy but address an orthogonal modality: multi-layer geometric imagery requiring spatial reasoning over proprietary rule semantics, rather than source code.
%To the best of our knowledge, no prior work aligns VLMs with VLSI layout geometry for signoff-level violation understanding and repair on multi-layer layouts from real design scenarios.

% \noindent\textbf{Spatial Reasoning in Vision-Language Models.}
% General-purpose VLMs perform well on natural-image VQA but exhibit significant spatial reasoning limitations. SpatialVLM~\cite{SpatialVLM} shows that synthetic spatial QA data can substantially enhance quantitative spatial understanding, while iVISPAR~\cite{iVISPAR} reveals that even SOTA VLMs fall short of human performance on multi-step spatial configurations.
%These findings motivate our approach: if VLMs require targeted spatial augmentation even for natural images, the gap is far more acute for VLSI layouts, where geometries are defined at nanometer precision, spatial semantics are governed by proprietary design rules rather than natural-world physics, and multi-layer interactions create topological constraints absent in natural scenes. Bridging this domain gap demands both domain-adapted training and a scalable source of signoff-verified layout--violation data—the bottleneck our self-supervised generation pipeline addresses.

% \noindent\textbf{Layout Pattern Generation.}
% Generating legal layout patterns is fundamental for DFM studies~\cite{VTS, VIPER, deesign_rule_manual, OPC_Pat_gen}. CNN~\cite{Deepattern} and GAN~\cite{CUP, CUP-EUV} approaches struggled with polygon-level constraints; LayouTransformer~\cite{LayouTransformer} improved legality via sequential token prediction; and diffusion models—DiffPattern~\cite{Diffpattern}, ControLayout~\cite{ControLayout}, PatternPaint~\cite{PatternPaint}, Vario~\cite{Vario, DiffLayoutDFM}—further advanced pattern diversity at sub-3nm nodes. However, these methods predominantly operate on rasterized single-layer images and cannot model cross-layer rule interactions (e.g., via enclosure, double-patterning) critical to multi-layer interconnects. Code-Not-Canvas~\cite{CodeNotCanvas} explored multi-agent LLM scripting for layout generation, but its script-based nature cannot learn from real layout distributions to reproduce complex, context-dependent violation scenarios.
% In contrast, our pipeline serializes multi-layer geometry into text and trains an autoregressive model with a self-supervised masked-prediction objective conditioned on real BEOL context and natural-language rule constraints, enabling controllable multi-layer generation with higher structural diversity than both diffusion-based and scripting baselines.

% In summary, the gaps identified above (text/code-only EDA agents, limited VLM spatial reasoning, and single-layer pattern generators) motivate our end-to-end framework: a self-supervised data generation pipeline that produces signoff-verified, multi-layer layout--violation pairs targeting complex conditional rules specified in flexible text, coupled with domain-adapted VLM fine-tuning that translates this geometric understanding into actionable guidance for local P\&R DRV fixing.
\vspace{-10pt}
\section{Related Work}

\noindent\textbf{LLMs and VLMs for EDA.}
LLMs have been widely adopted for text- and code-centric EDA tasks, including document and log QA~\cite{ORAssistant, DocumentQA_ICCAD, wan2025schemacoder}, chip design assistance~\cite{liu2023chipnemo}, RTL generation~\cite{ho2025verilogcoder, ScaleRTL, CraftRTL}, formal verification~\cite{wan2026fvrulelearner}, and multi-task reasoning~\cite{ho2026polymath}.
For design rule understanding, DRC-Coder~\cite{DRCCoder} and Rule2DRC~\cite{kim2026rule2drc} combine VLMs and LLMs to generate DRC checker code from rule descriptions before any violation occurs, whereas to our knowledge no prior work uses a VLM to visually ground a flagged violation, diagnose its root cause, and guide an agent to repair it.


% \noindent\textbf{Spatial Reasoning in Vision-Language Models.}
% General-purpose VLMs perform well on natural-image VQA but exhibit significant spatial reasoning limitations~\cite{SpatialVLM, iVISPAR}. This gap is far more acute for VLSI layouts, where geometries are defined at nanometer precision and spatial semantics are governed by proprietary design rules rather than natural-world physics—demanding both domain-adapted training and a scalable source of signoff-verified layout--violation data, the bottleneck our self-supervised generation pipeline addresses.

% \noindent\textbf{Layout Pattern Generation.}
% Generating legal layout patterns is fundamental for DFM studies~\cite{VTS, VIPER, deesign_rule_manual, OPC_Pat_gen}. CNN~\cite{Deepattern}, GAN~\cite{CUP, CUP-EUV}, token-based~\cite{LayouTransformer}, and diffusion~\cite{Diffpattern, ControLayout, PatternPaint, Vario, DiffLayoutDFM} methods have advanced pattern diversity, but operate on rasterized single-layer images and cannot model cross-layer rule interactions critical to multi-layer interconnects. Code-Not-Canvas~\cite{CodeNotCanvas} explored LLM scripting but cannot learn from real layout distributions.
% In contrast, our pipeline serializes multi-layer geometry into text and trains an autoregressive model with a self-supervised masked-prediction objective conditioned on real BEOL context and natural-language rule constraints, yielding higher structural diversity than both baselines.

% In summary, the gaps above (text/code-only EDA agents, limited VLM spatial reasoning, and single-layer pattern generators) motivate our framework: a self-supervised pipeline producing signoff-verified, multi-layer layout--violation pairs from flexible text-specified rules, coupled with VLM fine-tuning that translates geometric understanding into guidance for local P\&R DRV fixing.

% \noindent\textbf{Spatial Reasoning in Vision-Language Models.}
%General-purpose VLMs excel on natural-image VQA but struggle with spatial reasoning~\cite{SpatialVLM, iVISPAR}, especially for VLSI layouts where nanometer-precision geometries are governed by proprietary design rules. This demands domain-adapted training on scalable signoff-verified layout--violation data, which our self-supervised pipeline provides.

\noindent\textbf{Spatial Reasoning in VLMs.}
General-purpose VLMs struggle with spatial reasoning~\cite{SpatialVLM, iVISPAR}, especially for VLSI layouts governed by proprietary nanometer-precision rules, motivating domain-adapted training on DRC-annotated layout--violation data.

\noindent\textbf{Layout Pattern Generation.}
Prior CNN~\cite{Deepattern}, GAN~\cite{CUP, CUP-EUV}, token~\cite{LayouTransformer}, and diffusion~\cite{Diffpattern, ControLayout, PatternPaint, Vario, DiffLayoutDFM} methods advance DFM pattern diversity~\cite{VTS, VIPER, deesign_rule_manual, OPC_Pat_gen} but are limited to single-layer rasterized images. Our stage serializes multi-layer geometry into text, trains via self-supervised masked prediction from BEOL context, and steers generation with natural-language constraints at inference, capturing cross-layer diversity.

In summary, these gaps motivate our framework: a self-supervised layout-generation stage producing DRC-annotated multi-layer layout--violation pairs, coupled with VLM fine-tuning that provides actionable guidance for local P\&R DRV fixing.


==> VLM_ALIGN_DRC_ARXIV/tex/3_methods_v1.tex <==
\vspace{-10pt}
\section{Methodology}
% \vspace{-4pt}
% \input{figtexs/LayRep}
We propose a two-phase framework (Fig.~\ref{fig:proposed_framework}) that aligns VLMs with VLSI geometry to enable automated local P\&R DRV fixing. Section~3.1 describes our self-supervised data generation pipeline and VLM supervised fine-tuning for a domain-adapted DRC model (DRC-VLM); Section~3.2 describes the DRC-VLM-guided agentic framework for local P\&R DRV fixing; and Section~3.3 discusses why the two phases use different model modalities.

\vspace{-6pt}
\iffalse
\subsection{Phase~I: Self-Supervised Layout Generation \& VLM Supervised Fine-Tuning}

Phase~I is designed to close the data-scarcity and domain-gap barriers in two steps. Section~\ref{sec:layout_gen} trains an autoregressive model to generate diverse, signoff-verified layout--violation pairs from real designs. Section~\ref{sec:vlm_sft} curates multi-modal supervision from this corpus and uses it to fine-tune a domain-adapted DRC-VLM.

\subsubsection{Autoregressive Layout Generation Model}
\label{sec:layout_gen}
We design the pipeline to operate on production GDS files through four stages: (1)~tile the design into crops and rasterize each layer; (2)~extract connected components and serialize into a text representation; (3)~generate target-layer \texttt{[Poly]} sequences conditioned on context and optional text constraints; (4)~decode generated tokens into physical polygons, insert into the original layout, and run industrial DRC for rule annotation. This produces a signoff-verified, rule-annotated corpus anchored in real routed-layout topology.

\noindent\textbf{Text-Formulated Layout Representation.}
We propose a text-formulated, multi-layer layout representation (Fig.~\ref{fig:proposed_framework}) as the key enabler. Inspired by LayouTransformer~\cite{LayouTransformer}, we serialize each layout crop into structured tokens preserving layer identity, absolute position, and polygon extent. Each rectangle is encoded as a directional edge walk from its top-left vertex $(x,y)$ via cardinal deltas ($\rightarrow$~width, $\downarrow$~height, $\leftarrow$~width, $\uparrow$~height). The representation uses:
\begin{itemize}[nosep,topsep=0pt,leftmargin=*]
  \item \textbf{Layer headers} \texttt{[M1]}, \texttt{[M2]}, \texttt{[V1]} etc.: delimit each metal or via layer section.
  \item \textbf{\texttt{[Poly]}~\ldots~\texttt{[\textbackslash Poly]}}: a complete polygon fully contained within the crop window.
  \item \textbf{\texttt{[BPoly]}~\ldots~\texttt{[\textbackslash BPoly]}} (Boundary Polygon): a shape clipped by the crop boundary, used only as context, never as a generation target.
  \item \textbf{Coordinate tokens} $(x,\,y)$: absolute top-left vertex position in layout units.
  \item \textbf{Direction deltas} $\rightarrow w$, $\downarrow h$, $\leftarrow w$, $\uparrow h$: cardinal steps tracing the rectangle boundary.
\end{itemize}
This encoding is compatible with standard language-model training while preserving geometry needed for signoff-quality DRC annotation. We introduce the boundary-aware \texttt{[BPoly]} token to separate complete targets from context-only boundary shapes, ensuring the model does not treat clipped boundary shapes as valid generation targets or hallucinate geometry at crop edges.
% \textcolor{red}{Todo: This encoding is compatible with standard language-model training while preserving geometry needed for signoff-quality DRC annotation. Because both text coordinates and rendered axis annotations are expressed in absolute physical units, the model's geometric reasoning (e.g., spacing and enclosure measurements) is invariant to the crop window size. We introduce the boundary-aware \texttt{[BPoly]} token to separate complete targets from context-only boundary shapes, preventing the model from placing VIAs on partially visible metal stubs or hallucinating geometry at crop edges.}



\noindent\textbf{Self-Supervised Training \& Controllable Sampling.}
Let $X=\mathrm{Tok}(\mathcal{L}_{\mathrm{ctx}})$ denote the serialized context (both \texttt{[Poly]} and \texttt{[BPoly]}), $Y=(y_1,\ldots,y_T)=\mathrm{Tok}(\mathcal{L}_{\mathrm{gen}})$ the generated layer sequence (only \texttt{[Poly]}), and $C$ an optional text constraint describing the target rule family. The model factorizes as:
\vspace{-6pt}
\[
p_{\theta}(Y \mid X, C)
= \prod_{t=1}^{T} p_{\theta}(y_t \mid y_{<t}, X, C).
\]
\vspace{-8pt}

\noindent Training minimizes teacher-forced negative log-likelihood:
\vspace{-6pt}
\[
\mathcal{L}_{\mathrm{SFT}}(\theta)
= - \sum_{(X,Y,C)\in\mathcal{D}}
  \sum_{t=1}^{T} \log p_{\theta}(y_t \mid y_{<t}, X, C).
\]
\vspace{-8pt}

\noindent At inference, we sample tokens with temperature $\tau$:
\vspace{-6pt}
\[
y_t \sim \operatorname{softmax}\!\left(\frac{\mathbf{z}_t}{\tau}\right),
\quad
\mathbf{z}_t=f_{\theta}(y_{<t},X,C),
\]
\vspace{-8pt}

\noindent where larger $\tau$ increases diversity and the likelihood of rare rule-triggering configurations. We decode sampled sequences back into polygons and insert them into the original layout; signoff DRC labels each candidate as $(\hat{\mathcal{L}}, r, b)$ with violated rule $r$ and location $b$.
\fi

\subsection{Phase~I: Self-Supervised Layout Generation \& VLM Supervised Fine-Tuning}
% Phase~I is designed to close the data-scarcity and domain-gap barriers in two steps. Section~\ref{sec:layout_gen} trains an autoregressive model to generate diverse, signoff-verified layout--violation pairs from real designs. Section~\ref{sec:vlm_sft} curates multi-modal supervision from this corpus and uses it to fine-tune a domain-adapted DRC-VLM.

Phase~I is designed to close the data-scarcity and domain-gap barriers in two steps. Section~\ref{sec:layout_gen} trains an autoregressive model to generate diverse, DRC-annotated layout--violation pairs from real designs. Section~\ref{sec:vlm_sft} curates multi-modal supervision from this corpus and uses it to fine-tune a domain-adapted DRC-VLM.


\subsubsection{Autoregressive Layout Generation Model}
\label{sec:layout_gen}
% We design the pipeline to operate on production GDS files through four stages: (1)~tile the design into crops and rasterize each layer; (2)~extract connected components and serialize into a text representation; (3)~generate target-layer \texttt{[Poly]} sequences conditioned on context and optional text constraints; (4)~decode generated tokens into physical polygons, insert into the original layout, and run industrial DRC for rule annotation. This produces a signoff-verified, rule-annotated corpus anchored in real routed-layout topology.
We design the pipeline to operate on production GDS files through four stages: (1)~tile the design into crops and rasterize each layer; (2)~extract connected components and serialize into a text representation; (3)~generate target-layer \texttt{[Poly]} sequences conditioned on context and optional text constraints; (4)~decode generated tokens into physical polygons, insert into the original layout, and run industrial DRC for rule annotation. This produces a DRC-annotated, rule-labeled corpus anchored in real routed-layout topology.

\noindent\textbf{Text-Formulated Layout Representation.}
We propose a text-formulated, multi-layer layout representation (Fig.~\ref{fig:proposed_framework}) as the key enabler. Inspired by LayouTransformer~\cite{LayouTransformer}, we serialize each layout crop into structured tokens preserving layer identity, absolute position, and polygon extent. Each rectangle is encoded as a directional edge walk from its top-left vertex $(x,y)$ via cardinal deltas ($\rightarrow$~width, $\downarrow$~height, $\leftarrow$~width, $\uparrow$~height). The representation uses:
\begin{itemize}[nosep,topsep=0pt,leftmargin=*]
  \item \textbf{Layer headers} \texttt{[M1]}, \texttt{[M2]}, \texttt{[V1]} etc.: delimit each metal or via layer section.
  \item \textbf{\texttt{[Poly]}~\ldots~\texttt{[\textbackslash Poly]}}: a complete polygon fully contained within the crop window.
  \item \textbf{\texttt{[BPoly]}~\ldots~\texttt{[\textbackslash BPoly]}} (Boundary Polygon): a shape clipped by the crop boundary, used only as context, never as a generation target.
  \item \textbf{Coordinate tokens} $(x,\,y)$: absolute top-left vertex position in layout units.
  \item \textbf{Direction deltas} $\rightarrow w$, $\downarrow h$, $\leftarrow w$, $\uparrow h$: cardinal steps tracing the rectangle boundary.
\end{itemize}
This encoding is compatible with standard language-model training while preserving geometry needed for signoff-quality DRC annotation. We introduce the boundary-aware \texttt{[BPoly]} token to separate complete targets from context-only boundary shapes, ensuring the model does not treat clipped boundary shapes as valid generation targets or hallucinate geometry at crop edges.
% \textcolor{red}{Todo: This encoding is compatible with standard language-model training while preserving geometry needed for signoff-quality DRC annotation. Because both text coordinates and rendered axis annotations are expressed in absolute physical units, the model's geometric reasoning (e.g., spacing and enclosure measurements) is invariant to the crop window size. We introduce the boundary-aware \texttt{[BPoly]} token to separate complete targets from context-only boundary shapes, preventing the model from placing VIAs on partially visible metal stubs or hallucinating geometry at crop edges.}



\noindent\textbf{Self-Supervised Training \& Controllable Sampling.}
Let $X=\mathrm{Tok}(\mathcal{L}_{\mathrm{ctx}})$ denote the serialized context (both \texttt{[Poly]} and \texttt{[BPoly]}) and $Y=(y_1,\ldots,y_T)=\mathrm{Tok}(\mathcal{L}_{\mathrm{gen}})$ the generated layer sequence (only \texttt{[Poly]}). During training, the model learns to reconstruct masked polygons from context alone:
\vspace{-6pt}
\[
p_{\theta}(Y \mid X)
= \prod_{t=1}^{T} p_{\theta}(y_t \mid y_{<t}, X).
\]
\vspace{-8pt}

\noindent Training minimizes teacher-forced negative log-likelihood:
\vspace{-6pt}
\[
\mathcal{L}_{\mathrm{SFT}}(\theta)
= - \sum_{(X,Y)\in\mathcal{D}}
  \sum_{t=1}^{T} \log p_{\theta}(y_t \mid y_{<t}, X).
\]
\vspace{-8pt}

\noindent At inference, we augment the context with an optional natural-language constraint $C$ describing the target rule family (e.g., ``generate more tip-to-tip M$x$ shapes'' or ``target VIA spacing violations'') and sample tokens with temperature $\tau$:
\vspace{-6pt}
\[
y_t \sim \operatorname{softmax}\!\left(\frac{\mathbf{z}_t}{\tau}\right),
\quad
\mathbf{z}_t=f_{\theta}(y_{<t},X,C),
\]
\vspace{-8pt}

% \noindent where larger $\tau$ increases diversity and the likelihood of rare rule-triggering configurations. We decode sampled sequences back into polygons and insert them into the original layout; signoff DRC labels each candidate as $(\hat{\mathcal{L}}, r, b)$ with violated rule $r$ and location $b$.
\noindent where larger $\tau$ increases diversity and the likelihood of rare rule-triggering configurations. Constraint following relies on the instruction-following capability of the pretrained language model; layout fine-tuning teaches only the structured polygon representation, leaving the model's ability to condition on natural-language prompts intact. We decode sampled sequences back into polygons and insert them into the original layout; signoff DRC checker then annotates each candidate with the violated rule and violation location.
% \noindent where larger $\tau$ increases diversity and the likelihood of rare rule-triggering configurations. Constraint following relies on the instruction-following capability of the pretrained language model; layout fine-tuning teaches only the structured polygon representation, leaving the model's ability to condition on natural-language prompts intact. We decode sampled sequences back into polygons and insert them into the original layout; signoff DRC labels each candidate as $(\hat{\mathcal{L}}, r, b)$ with violated rule $r$ and location $b$.
\input{tabtex/DataComposition}

\subsubsection{VLM Supervised Fine-Tuning for Local DRV}
\label{sec:vlm_sft}
We run a DRC checker~\cite{Calibre} on the generated layout crops from Section~\ref{sec:layout_gen} to obtain ground-truth violation labels and locations, which we then curate into two complementary multi-modality supervision categories (Table~\ref{tab:data_composition}):
\begin{itemize}[nosep,topsep=2pt,leftmargin=*]
\item \textbf{DRC Analysis Task:} A teacher model
  (Gemini-3-Pro) receives each layout crop image together with its
  DRC violation report and generates a reasoning trace that
  identifies relevant layout features, measures dimensions, compares
  against rule thresholds, and concludes with the violated rule. We
  apply multi-stage filtering on rule coverage, violation polygon
  location, and direction/spacing consistency, removing
  13.40\% of traces with image input
  (Table~\ref{tab:filter_stage}).
%\textcolor{blue}{We provide the DRC violation report and the image to a teacher model (Gemini-3-Pro), which generates reasoning traces that identify layout features, measure dimensions, compare against thresholds, and conclude with the violated rule. The traces undergo multi-stage filtering: samples are removed if rule coverage is below 80\%, predicted violation polygons do not match ground-truth locations, or the reasoning contains inconsistent direction or spacing measurements. Approximately 13\% of traces are filtered out with the details in Section~\ref{Sec:ModalityDiscuss}.}
\item \textbf{Description Task:} We pair each crop with programmatically extracted metal shape and VIA center coordinates in a structured JSON response, teaching the model to perceive, count, and localize geometric features.
\end{itemize}

We combine both data categories into a unified, shuffled training mixture for supervised fine-tuning of Qwen3-VL-8B~\cite{Qwen3VL}. Each sample pairs a layout crop and rule description with either a structured JSON prediction or a reasoning trace followed by the prediction. We train the model with autoregressive cross-entropy loss over target tokens (prompt and image tokens masked), jointly optimizing layout perception, violation classification, and diagnostic reasoning.
% Only language-model parameters are updated to preserve pretrained visual representations. Training hyperparameters are detailed in Section~\ref{Sec:VLMSFTExp}.


\vspace{-4pt}
\subsection{Phase II: VLM-Guided Local P\&R DRV Fixing}

We employ the domain-adapted DRC-VLM as an expert diagnostic front-end to a SOTA AI agent for local P\&R DRV repair (Fig.~\ref{fig:proposed_framework}).
We input the DRC-VLM with a rendered image of the local layout region, the DRC error report, and the relevant design-rule description; it produces a structured expert analysis: root-cause identification, the specific polygons involved with their coordinates, and a ranked list of top-$k$ potential fix actions with predicted connectivity impact.

This analysis is then provided to a SOTA AI coding agent equipped with DRC and LVS checker tools.
%The agent directly edits the local GDS without a predefined action space or fix-template vocabulary: it may move, resize, add, or remove metal and via polygons on the target layers as needed to resolve the violation, with the sole constraint that boundary polygons shared with the surrounding design context remain unmodified.
The agent directly edits the local GDS without a predefined action space: it may move, resize, add, or remove interior polygons as needed, while boundary polygons may only be extended or supplemented, not removed, to preserve connectivity with the surrounding design.
DRC and LVS checkers are invoked after every edit to verify rule legality and preserve circuit connectivity, forming a checker-in-the-loop repair cycle.
Unlike template-based engines that narrow the search space through static, pre-encoded correction patterns, the DRC-VLM provides dynamic, rule-conditioned guidance grounded in domain knowledge of complex conditional design rules, enabling the agent to adapt its fixes to each violation's geometric and topological context.

\subsection{Discussion: Choosing the Model Modality}
\label{Sec:ModalityDiscuss}

%\todo{
%We use a text LLM for layout augmentation because our structured representation enables diverse outputs that decode directly into editable polygons. Image-based generation instead requires vectorization, grid snapping, layer assignment, and filtering or repair before signoff, reducing the yield of valid samples.
%}
%\todo{
%DRC reasoning, however, requires understanding spatial relations such as spacing, enclosure, and multi-layer interactions. Layout images expose these relations directly, whereas polygon sequences flatten two-dimensional topology into a long token stream. Our experiments therefore support complementary modalities: text for controllable layout generation and vision for spatial DRC analysis.
%}

We use a text LLM for layout augmentation because our structured
representation enables diverse outputs that decode directly into
editable polygons, whereas image-based generation would require
vectorization, grid snapping, layer assignment, and filtering before
signoff. DRC reasoning, however, demands understanding of spatial
relations such as spacing, enclosure, and multi-layer interactions
that layout images expose directly but polygon sequences flatten into
long token streams. To validate this, we compare the filtering rates
of reasoning traces generated from text-represented layouts versus
image inputs on the DRC Analysis Task
(Table~\ref{tab:filter_stage}). 
Text input leads to a 30.66\%
overall filtering rate versus only 13.40\% for image input, with the
gap concentrated at the location stage (21.60\% vs.\ 3.50\%): the
text representation enables correct rule identification and logically
valid reasoning, yet lacks the spatial context to distinguish the
exact violating polygon from geometrically identical neighbors. These
results confirm complementary roles for the two modalities, text for
controllable layout generation and vision for spatial DRC analysis,
and demonstrate that visual input is irreplaceable for polygon-level
localization in dense layouts.
%\input{figtexs/FixingFlow}

\begin{table}[h]
\centering
\caption{Filtering rate of reasoning traces at each stage for text-represented layout versus image input on the DRC Analysis Task.}
\label{tab:filter_stage}
\small
\begin{tabular}{lcccc}
\hline
 & \multicolumn{4}{c}{Filter Stage} \\
\cline{2-5}
 & DRV Rule & Location & Dir./Measure & Total \\
\hline
Text Rep. & 4.03\% & 21.60\% & 5.03\% & 30.66\% \\
Image     & 9.60\% & 3.50\%  & 0.30\% & 13.40\% \\
\hline
\end{tabular}
\end{table}

==> VLM_ALIGN_DRC_ARXIV/tex/4_experiments.tex <==
\vspace{-6pt}
\section{Experimental Results}\label{sec:experiments}
%We evaluate our framework along three axes: layout data generation quality, DRV detection and understanding, and local DRC fixing at an advanced technology node. The framework is implemented in Python. The auto-regressive layout generation model (Qwen2.5-3B-Instruct) and the DRC-VLM (Qwen3-VL-8B) are fine-tuned using NVIDIA Megatron-LM~\cite{Megatron} through the NeMo framework with tensor parallelism (TP\,=\,4) across 4$\times$ NVIDIA A100-80GB GPUs on a single node. Both models use the Adam optimizer ($\beta_1$\,=\,0.9, $\beta_2$\,=\,0.95) with a cosine learning rate schedule (peak LR\,=\,$5{\times}10^{-6}$, min LR\,=\,$5{\times}10^{-7}$) and 150 warmup iterations.
%For the DRV rule set, we select a subset of place-and-route-relevant DRC rules from the thousands available at the sub-2\,nm technology node, covering spacing, enclosure, color spacing, group via spacing, and width constraints.
Our evaluation covers layout data generation quality, DRV detection and understanding, and local DRV fixing at an advanced technology node.
Both the auto-regressive layout generation model (Qwen2.5-3B-Instruct) and DRC-VLM (Qwen3-VL-8B) are fine-tuned using AdamW ($\beta_1$\,=\,0.9, $\beta_2$\,=\,0.95) with a cosine learning-rate schedule on 4$\times$ A100-80GB GPUs.
For the DRV rule set, we select a subset of local P\&R relevant DRC rules from the thousands available at the sub-2\,nm technology node, covering spacing, enclosure, color spacing, group via spacing, and width constraints.

\input{tabtex/layoutGen}
\input{figtexs/Coverage}
\subsection{DRV Layout Data Generation Evaluation}

%We evaluate the quality of the generated DRC violation layout dataset. The auto-regressive layout generation model is trained on 1,000 real design layout crops paired with textual constraints specifying layer parameters and target DRV conditions. During inference, we randomly mask local metal and via routing shapes and condition the model on text constraints under high-temperature sampling to generate diverse DRV layouts.
%The text constraints can be rule specific or geometric related, such as generate more via groups, more tip-to-tip Mx shape, etc.
We evaluate the quality of the generated DRC violation layout dataset. The auto-regressive layout generation model is trained on 1,000 real design layout crops using random polygon masking and reconstruction from BEOL context alone, without constraints or violation labels. During inference, we supply rule-specific or geometric constraints (e.g., generate more VIA groups, more tip-to-tip M$x$ shapes) and sample under high temperature to steer generation toward violation-prone configurations.
% We evaluate the quality of the generated DRC violation layout dataset. The auto-regressive layout generation model is trained on 1,000 real design layout crops paired with textual constraints specifying layer parameters and target DRV conditions. During inference, we randomly mask local metal and via routing shapes and condition the model on text constraints under high-temperature sampling to generate diverse DRV layouts.
% The text constraints can be rule specific or geometric related, such as generate more via groups, more tip-to-tip Mx shape, etc.
Each method generates ${\sim}$15K samples; after filtering out-of-scope and near-duplicate DRVs, these are used for the downstream VLM training comparison in Section~\ref{Sec:VLMSFTExp}.
% \textcolor{red}{Need to provide examples of the text constraints?}

\noindent\textbf{Baselines.}
% We compare against two baselines: a discrete diffusion model (D3PM)~\cite{PatternPaint} trained on the same data, and an agentic script-based method in which a SOTA coding agent~\cite{claudecode2026} is provided with DRC rule descriptions and layer parameters (preferred routing direction, pitch, and width) to generate Python scripts for DRV layout creation.
We compare against two baselines: a discrete diffusion model (D3PM)~\cite{PatternPaint} trained on the same data, and an agentic script-based method in which a SOTA coding agent~\cite{claudecode2026} is provided with DRC rule descriptions and layer parameters (routing directions, pitch, and width) to generate Python scripts. These scripts are then executed to produce synthetic DRV layout--violation pairs.



\noindent\textbf{Evaluation Metrics and Results.}
We measure generation quality using layout entropy ($H$)~\cite{Deepattern, LayouTransformer}, unique topologies, and validated triggered design rules, as shown in Table~\ref{tab:dataset_metrics}. Following~\cite{LayouTransformer}, $H$ is the Shannon entropy over scan-line counts $(c_x,c_y)$:
\vspace{-4pt}
\[
H = - \sum_i \sum_j P(c_{x_i}, c_{y_j}) \log P(c_{x_i}, c_{y_j}).
\]
\vspace{-6pt}

\input{figtexs/SFTPredictionTask}

\noindent Unique topologies are distinct $(c_x,c_y)$ pairs; rule coverage counts validated triggered rules after filtering out-of-scope and near-duplicate DRVs.
Our method achieves the highest entropy ($H=5.07$), the most unique layouts (289), and the broadest validated rule coverage, triggering 29 VIA and 34 metal rule types. The t-SNE visualization in Fig.~\ref{fig:tsne_coverage}, further confirms that the auto-regressive generator and D3PM match the geometric distribution of real routed layouts, while the agentic script baseline produces simpler patterns that deviate from real designs.


% We measure generation quality using layout entropy ($H$)~\cite{Deepattern, LayouTransformer}, unique topologies, and validated triggered design rules, as shown in Table~\ref{tab:dataset_metrics}. Following~\cite{LayouTransformer}, $H$ is the Shannon entropy of the joint pattern-complexity distribution over $(c_x,c_y)$, where $c_x$ and $c_y$ are the numbers of scan lines along the $x$- and $y$-axes minus one:
%\[
%H = - \sum_i \sum_j P(c_{x_i}, c_{y_j}) \log P(c_{x_i}, c_{y_j}).
%\]
%Unique topologies are counted as distinct $(c_x,c_y)$ pairs. For DRC rule coverage, we filter out violations outside the selected rule set and remove near-duplicate DRV samples before counting validated triggered rules.

%Our method achieves the highest entropy ($H=5.07$), the most unique layouts (289), and the broadest validated rule coverage, triggering 29 VIA and 34 metal rule types. The t-SNE visualization in Fig.~\ref{fig:tsne_coverage}, further confirms that the auto-regressive generator and D3PM match the geometric distribution of real routed layouts, while the agentic script baseline produces simpler patterns that deviate from real designs.

% \input{figtexs/Dataset_Aug}



\vspace{-10pt}
% \input{tabtex/Ablation1_DataScaling}
\subsection{VLM Supervised Fine-Tuning Result} \label{Sec:VLMSFTExp}

The DRV detection task is designed to strengthen the model's understanding of layout geometry and design-rule constraints as shown in Fig.~\ref{fig:sftinputexample}. Unlike simple object localization, this task requires the VLM to reason about spatial relationships between polygons, measure rule-relevant distances, and identify violation-causing regions. This provides high-value supervision for downstream layout tasks, which are diverse, scenario-dependent, and difficult to exhaustively construct as training data. 


\begin{table}[!t]
\centering
\caption{DRV detection testing dataset rule frequency by category.}
\label{tab:benchmark_statistics}
\scriptsize
\begin{tabular}{lcc}
\toprule
\textbf{VIA / Metal Category} & \textbf{VIA (100 samples)} & \textbf{Metal (100 samples)} \\
\midrule
W / W+A        & 5   & 180 \\
Spc            & 177 & 108 \\
EN             & 3   & 81  \\
G-Spc / R      & 308 & 25  \\
Grp / CS       & 30  & 15  \\
G-Spc / EN     & 308 & 81  \\
\midrule
Total triggers & 523 & 409 \\
Avg./sample    & 5.23 & 4.09 \\
\bottomrule
\end{tabular}
\end{table}

\input{tabtex/SFTResultTable}
\input{tabtex/DRVFixTable}

\noindent\textbf{Training Data Composition.}
Table~\ref{tab:data_composition} summarizes the training data. After filtering DRC violations and removing near-duplicate tasks, our proposed pipeline yields 16,861 VIA and 17,254 metal samples spanning DRC analysis (with both reasoning and non-reasoning supervision) and layout description tasks (via counting, localization, and bounding-box extraction). As a baseline, we collect 15,499 VIA and 16,749 metal samples using script-based generation with the same filtering procedures.

% \noindent\textbf{DRV Detection Testing Dataset.}
%We construct a 200-sample testing dataset (100 VIA, 100 metal) from an unseen design layout crops. Each sample may contain multiple co-occurring violations, requiring models to identify all violated rules and localize every violation instance. As shown in Table~\ref{tab:benchmark_statistics}, the testing dataset contains 523 VIA-rule and 409 metal-rule triggers (averages of 5.23 and 4.09 per sample), spanning width/area, spacing, enclosure, routing/restriction, group/color spacing, and combined spacing-enclosure constraints.

\noindent\textbf{DRV Detection Testing Dataset.}
We construct a 200-sample test set (100 VIA, 100 metal) from real layout crops of a \emph{different IP} than the training data; both share the same sub-2\,nm rule deck but have disjoint routing patterns. Each sample may contain multiple co-occurring violations; as shown in Table~\ref{tab:benchmark_statistics}, the set contains 523 VIA-rule and 409 metal-rule triggers (avg.\ 5.23 and 4.09 per sample) spanning categories mentioned in Table~\ref{tab:dataset_metrics}.


\noindent\textbf{Evaluation Metrics.}
Each response is scored at two levels: \emph{Rule identification} via set-level F1 between predicted and ground-truth violated-rule sets, and \emph{Localization}, gated by rule correctness—a prediction $(\hat{r},\hat{p})$ is a TP only if $\hat{r}$ matches a ground-truth rule and $\hat{p}$ matches its ground-truth location, else FP:
\vspace{-4pt}
\[
\text{Loc}(\hat{r}, \hat{p}) =
\begin{cases}
\mathrm{TP}, & \hat{r} \in \mathcal{R}_{\mathrm{GT}} \ \text{and}\  \hat{p} \leftrightarrow \mathcal{P}_{\mathrm{GT}}(\hat{r}),\\
\mathrm{FP}, & \text{otherwise},
\end{cases}
\]
\vspace{-6pt}

% \noindent Unmatched ground-truth instances count as FN. Each sample is evaluated over $n=10$ trials; following the unbiased pass@$k$ estimator of~\cite{chen2021evaluating}, we generalize it to continuous scores by computing the expected maximum F1 over all $\binom{n}{k}$ subsets of $k$ draws, averaged across 200 data samples. Rule F1 and Loc F1 are each aggregated this way, and Comb F1 is their harmonic mean.
\noindent Unmatched ground-truth instances count as FN. Each sample is evaluated over $n=10$ trials and aggregated via the pass@$k$ estimator~\cite{chen2021evaluating} for Rule F1 and Loc F1; Comb F1 is their harmonic mean.
% \noindent Unmatched ground-truth instances count as FN. Each sample is evaluated over $n=10$ trials and aggregated via the pass@$k$ estimator~\cite{chen2021evaluating} (expected maximum F1 over $k$ draws); Comb F1 is their harmonic mean of Rule F1 and Loc F1.
%Each sample is evaluated over 10 trials and aggregated via pass@$k$~\cite{chen2021evaluating} for Rule F1 and Loc F1; Comb F1 is their harmonic mean.


\noindent\textbf{Baselines.}
We compare against strong SOTA VLM baselines, including Gemini-3-Pro, GPT-5.2, and Qwen3-VL-8B-Base, using identical rule descriptions and layout images as input.



% \noindent\textbf{Evaluation Result.} Table~\ref{tab:combined_metal_via_results} shows that higher-quality generated training data directly improves VLM performance on DRV detection: our method achieves the best overall pass@5 Comb F1 of 44.2, a 24.8-point gain over the base model, versus 32.8 for Gemini-3-Pro. The gain is largest in localization—the script-based baseline (Mixed-NoR-Script) attains high Rule F1 but poor Loc F1, showing it exposes rule labels without the geometric fidelity needed for spatial grounding—confirming that realistic generated layouts are critical for accurate violation localization.
% This fine-tuned model, our domain-adapted DRC-VLM, is used next to guide local P\&R DRV fixing.
\input{figtexs/CaseStudy_Combined}
\noindent\textbf{Evaluation Result.} Table~\ref{tab:combined_metal_via_results} shows that higher-quality generated training data directly improves VLM performance on DRV detection: our method achieves the best overall pass@5 Comb F1 of 44.2, a 24.8-point gain over the base model, versus 32.8 for Gemini-3-Pro. The main bottleneck for general VLMs is localization rather than rule recall: Gemini-3-Pro reaches only 24.6 Loc F1 at pass@5, GPT-5.2 reaches 17.5, and Qwen3-VL-8B-Base reaches 12.4, despite receiving the same rule descriptions and layout images. The gain from our data is also largest in localization---the script-based baseline (Mixed-NoR-Script) attains high Rule F1 but poor Loc F1, showing it exposes rule labels without the geometric fidelity needed for spatial grounding---confirming that realistic generated layouts are critical for accurate violation localization.
This aligns with the filtering analysis in Section~\ref{Sec:ModalityDiscuss}: even Gemini-3-Pro, our teacher model, achieves only 24.6 Loc F1---it can generate reasoning traces but cannot reliably localize violating polygons, making fine-tuning on our DRC-annotated layout data essential for Phase~II guidance.
% This aligns with the filtering analysis in Section~\ref{Sec:ModalityDiscuss}: even Gemini-3-Pro, our teacher model, achieves only 24.6 Loc F1---it can generate reasoning traces but cannot reliably localize violating polygons, making fine-tuning on our signoff-verified layout data essential for Phase~II guidance.
As a result, our domain-adapted DRC-VLM is used next to guide local P\&R DRV fixing.


% Table~\ref{tab:combined_metal_via_results} shows that higher-quality generated training data directly improves VLM performance on DRV detection. Our proposed method achieves the best overall pass@5 combined score of 44.2, compared with 32.8 for Gemini-3-Pro and 19.4 for Qwen3-VL-8B-Base, a 24.8-point gain over the base model that demonstrates domain-specific layout generation provides supervision that general pretraining alone does not capture. The improvement is most evident in localization: on Metal, the proposed model reaches 44.6 Comb F1 at pass@5, while the script-based baseline (Mixed-NoR-Script) obtains high Rule F1 but poor Loc F1, indicating that script-generated layouts expose rule labels but lack the geometric fidelity needed for spatial grounding. On VIA, the proposed model similarly achieves the best pass@5 Comb F1 of 43.7. These results confirm that realistic generated layout data is critical for connecting rule understanding with accurate violation localization.
\vspace{-6pt}
\subsection{Local DRC Fixing Experiment}
We demonstrate that DRC-VLM can significantly improve SOTA AI agents on fixing local P\&R DRC violations at sub-2nm technology node.
Given that general VLMs fail at the prerequisite localization task (Table~\ref{tab:combined_metal_via_results}), we employ our domain-adapted DRC-VLM as the expert front-end.
% We demonstrate that DRC-VLM can significantly improve SOTA AI agents on fixing local P\&R DRC violations at an advanced technology node.
%We select a block-level design that was DRC-clean under prior design-rule deck but exhibits numerous DRC errors under the latest design-rule deck at a sub-2\,nm technology node.
For each DRV, we extract a local GDS region surrounding the violation site as the repair context.
% The agent may freely modify or remove interior polygons, but boundary polygons shared with the surrounding design context cannot be removed; the agent may only extend them or add new boundary-polygon segments within the local window, preserving connectivity beyond the repair scope.
Interior polygons may be freely edited, while boundary polygons may only be extended or supplemented, not removed, to preserve surrounding connectivity.
Given the target DRV error report, the local layout netlist, and a rendered image of the region, the fine-tuned DRC-VLM analyzes the violation and proposes an expert analysis including top-$k$ potential fixes, where $k=3$.
This expert analysis is then supplied to a SOTA coding agent equipped with DRC and LVS checker tools to fix the local DRVs.
We run the agent fix once per problem for both proposed method and baselines for a fair comparison.


\noindent\textbf{Local P\&R DRV Dataset.}
%We curate a 100 local P\&R DRV dataset by selecting representative error regions and filtering out duplicated or near-identical samples.
%The dataset spans a diverse mix of rule interactions rather than isolated single-rule edits:
%39 cases involve conditional via--metal enclosure,
%27 require metal or via width-quantization fixes,
%21 involve spacing interactions,
%10 target double-patterning color-spacing constraints,
%and 3 target minimum-area violations.
%The spacing cases further cover both same-layer metal spacing and cross-layer via interactions, making the dataset representative of local ECO scenarios in which geometric legality, connectivity preservation, and advanced-node design-rule context must all be satisfied simultaneously.
% From an unseen block-level IP design that was DRC-clean under a prior developing rule deck but exhibits numerous errors under the latest rule deck at sub-2nm, we curate 100 local P\&R DRV cases by selecting representative error regions and filtering duplicates. The dataset spans five categories (EN: 39, Width: 27, Spacing: 21, Color Spacing: 10, Area: 3) covering same-layer and cross-layer interactions, making it representative of local Engineering Change Order (ECO) scenarios where geometric legality, connectivity, and advanced-node context must all be satisfied.
From an unseen block-level IP design that was DRC-clean under a prior developing rule deck but exhibits numerous errors under the latest rule deck at sub-2nm, we curate 100 local P\&R DRV cases by selecting representative error regions and filtering duplicates. The dataset spans five categories (EN: 39, Width: 27, Spacing: 21, Color Spacing: 10, Area: 3) covering same-layer and cross-layer interactions, making it representative of local Engineering Change Order (ECO) scenarios where geometric legality, connectivity, and advanced-node context must all be satisfied.
Curation prioritizes hard-to-fix conditional rules (enclosure, color spacing); the category distribution matches the actual P\&R error distribution.
Each instance requires up to 1{,}800\,s of agent compute with iterative checker feedback, making large-scale evaluation costly; the Area category (3 cases) is included for completeness but is too small to draw per-category conclusions.

\noindent\textbf{Baselines.}
%We compare against two state-of-the-art coding agents~\cite{claudecode2026, OpenAICodex2026} \emph{without} the proposed expert analysis from DRC-VLM. Claude Code uses Sonnet~4.6~\cite{anthropic2026claude} as its core model, and Codex uses GPT-5.4~\cite{OpenAI_GPT54}. Each agent is provided with DRC rule descriptions, metal pitch and preferred routing direction parameters, and the input GDS and rendered layout image in a shared working directory. Both agents have access to DRC and LVS signoff checker tools, with an 1800\,s time limit imposed per DRV fixing instance.
We compare against two SOTA coding agents~\cite{claudecode2026, OpenAICodex2026} \emph{without} the proposed expert analysis from DRC-VLM. Claude Code uses Sonnet~4.6~\cite{anthropic2026claude} as its core model, and Codex uses GPT-5.4~\cite{OpenAI_GPT54}. Each agent is provided with DRC rule descriptions, metal pitch and preferred routing direction parameters, the raw DRC report, the input GDS, and the rendered PNG layout image in a shared working directory. Both agents have access to DRC and LVS signoff checker tools, with an 1800\,s time limit imposed per DRV fixing instance.
These constitute strong baselines: as SOTA coding agents, they can programmatically analyze DRC reports, restructure rule and layout information, inspect rendered images, and iteratively repair the GDS with checker-in-the-loop feedback.



\noindent\textbf{Evaluation Metrics.}
A case is \emph{solved} if the target DRV is fixed without introducing new DRVs in the region \emph{and} the design passes LVS. We report the solve rate per category and overall.


%\noindent\textbf{Experiment Results.}
%Table~\ref{tab:drc_combined} (left) reports the local DRV fixing results on the 100-case DRV fixing dataset across five DRV rule categories.
%The baseline rows use the coding agents alone, while the proposed rows augment %each agent with DRC-VLM guidance that provides rule-aware visual context during repair.
%Each category entry shows the number of solved cases and the corresponding solve rate; the absolute SR improvement over the respective baseline is shown below each value in green.
%DRC-VLM-assisted methods consistently improve fixing performance across all categories: with DRC-VLM expert analysis, Claude Code's overall solve rate increases from 63.0\% to 88.0\%, and Codex's from 85.0\% to 97.0\%.
%Figure~\ref{fig:case_study} illustrates representative examples of DRV fixing by the baseline agents and the proposed DRC-VLM agentic method.
%Without knowledge of the proprietary conditional patterning and spacing rules, the baseline agents struggle to resolve local DRVs without introducing new violations.
%By contrast, the DRC-VLM model, trained on conditional design rules and geometric relations, provides structured analysis including root cause, potential fixes, and connectivity impact, enabling the agents to successfully repair the target DRVs without cascading errors.
%\textcolor{blue}{The remaining unsolved cases are concentrated in the Color Spacing category,
%where violations arise in tight spacing interaction regions that risk triggering cascading enclosure violations, requiring net-level rerouting beyond the local repair scope.}

%\noindent\textbf{Token Cost Analysis.}
%Table~\ref{tab:drc_combined} (right) shows that DRC-VLM guidance reduces average token cost by 15.2\% for Claude Code and 2.2\% for Codex overall.
%The largest savings concentrate in rule-intensive categories: Color Spacing drops by 45.6\% for Claude Code, and EN decreases by 19.9\% and 4.6\% for Claude Code and Codex, respectively, reflecting fewer exploratory iterations when the agent receives rule-aware root-cause analysis upfront.


\noindent\textbf{Experiment Results.}
Table~\ref{tab:drc_combined} reports local DRV fixing results (left) and token cost (right) across five rule categories on the 100-case dataset.
DRC-VLM-assisted methods consistently outperform the coding-agent baselines: Claude Code's overall solve rate rises from 63.0\% to 88.0\%, and Codex's from 85.0\% to 97.0\%.
Without knowledge of proprietary conditional rules, baseline agents struggle to resolve DRVs without introducing new violations; the DRC-VLM provides structured root-cause analysis, potential fixes, and connectivity impact, enabling successful repair without cascading errors.
As Figure~\ref{fig:case_study} illustrates, baseline agents attempt plausible but rule-unaware edits that trigger new violations, whereas DRC-VLM-guided agents apply rule-compliant corrections, confirming that explicit geometric reasoning is a stronger prior than iterative trial-and-error.
The remaining unsolved cases concentrate in the Color Spacing category, where tight spacing interactions risk triggering cascading violations that require net-level rerouting beyond the local repair scope.
% For token cost, DRC-VLM guidance reduces average tokens by 15.2\% for Claude Code and 2.2\% for Codex, with the largest savings in Color Spacing and EN categories, reflecting fewer exploratory iterations when the agent receives rule-aware analysis upfront.
For token cost, DRC-VLM guidance reduces average tokens by 24.5\% for Claude Code and 2.2\% for Codex, with the largest savings in Color Spacing and EN categories, reflecting fewer exploratory iterations when the agent receives rule-aware analysis upfront.

% \noindent\textbf{Experiment Results.}
%Table~\ref{tab:drc_combined} reports local DRV fixing results and token cost across five rule categories on the 100-case dataset.
%DRC-VLM-assisted methods consistently outperform the coding-agent baselines: Claude Code's overall solve rate rises from 63.0\% to 88.0\%, and Codex's from 85.0\% to 97.0\%.
%Without knowledge of proprietary conditional rules, baseline agents struggle to resolve DRVs without introducing new violations; the DRC-VLM model provides structured root-cause analysis, potential fixes, and connectivity impact, enabling successful repair without cascading errors (Figure~\ref{fig:case_study}).
%The remaining unsolved cases are concentrated in the Color Spacing category, where tight spacing interactions risk triggering cascading violations that require net-level rerouting beyond the local repair scope.
%On the token cost side, DRC-VLM guidance reduces average tokens by 15.2\% for Claude Code and 2.2\% for Codex, with the largest savings in rule-intensive categories---Color Spacing (45.6\%) and EN (19.9\%, 4.6\%)---reflecting fewer exploratory iterations when the agent receives rule-aware analysis upfront.


% To demonstrate the practical value of our domain-adapted model, we present two representative DRC fixing case studies (Fig.~\ref{fig:case_study}) comparing an agentic workflow without model-provided hints against the same agent augmented with diagnostic hints from our domain-adapted VLM. In the baseline workflow, the LLM agent (Gemini 2.5 Pro) directly attempts to fix the DRV from the layout without any domain-specific guidance. In our workflow, the trained domain-adapted VLM first analyzes the DRV to produce structured diagnostic insights (including root cause analysis and potential fix actions), which then guide the agent to perform the actual layout editing.

% The VLM proposes fix actions from a predefined vocabulary of layout editing primitives. Two key actions used in our case studies are: \texttt{extend\_metal}, which grows an existing M1/M2 rectangle along specified sides to improve enclosure margins (LVS-safe, as it only adds metal area); and \texttt{create\_local\_bridge\_metal\_via}, a compound action that removes an offending VIA, extends metal to bridge to a DRC-legal position, and places a replacement VIA to re-establish M1--M2 connectivity. Each fix step is annotated with its \emph{connectivity impact} (preserves, breaks, or re-establishes an M1--M2 connection) to maintain circuit-level correctness.

% \noindent\textbf{Spacing Rule (R2-S).}
% Fig.~\ref{fig:case_study} (top row) presents a scenario involving VIA1 spacing (VIA1 to VIA1 $\geq S_{\min}$) that requires consideration of the surrounding routing environment. The agent without hints naively adds a new via without considering the M2 routing context, introducing an additional DRV. Our domain-adapted VLM, however, precisely identifies the root cause: the two VIA1 instances at $(x_1, y_1)$ and $(x_2, y_2)$ are separated by only $d_{\mathrm{act}}$ edge-to-edge, well below the required $S_{\min}$ minimum. 
% It proposes a local bridge metal via action (\texttt{create\_local\_bridge\_metal\_via}) that relocates the problematic via while preserving LVS connectivity, allowing the agent to cleanly resolve the spacing violation.
% \textcolor{blue}{It proposes a \texttt{create\_local\_bridge\_metal\_via} action that relocates the problematic via using a bridge metal while maintaining LVS connectivity, and with this guidance, the agent cleanly resolves the spacing violation.}

% \noindent\textbf{Enclosure Rule (R4-EN).}
% Fig.~\ref{fig:case_study} (bottom row) illustrates a conditional enclosure violation: when M2 width $< W_t$, the M2 opposite enclosure must be $\geq E_{\min}$. The original layout contains 3 such violations. The agent without hints attempts to extend the M2 metal to increase enclosure, but fails to respect the M2 preferred routing direction and width constraints, introducing a new violation. In contrast, our domain-adapted VLM correctly identifies the root cause, insufficient M2 enclosure due to narrow wire widths ($E_{\mathrm{act}}$ vs.\ required $E_{\min}$), and proposes targeted \texttt{extend\_metal} actions along the proper routing directions. With these hints, the agent successfully resolves all violations.


% These case studies illustrate two complementary failure modes of direct agent baselines: \emph{rule-awareness} failures, where the agent proposes geometrically invalid repairs (e.g., extending metal along the wrong routing direction), and \emph{geometric reasoning} failures, where the agent misidentifies the root cause entirely (e.g., adding connectivity instead of relocating a VIA). Our diagnostic decomposition addresses both by providing the agent with precise measured deficiencies, rule-constrained fix actions, and coordinates of all involved features, reducing the search space from open-ended layout editing to targeted, rule-compliant modifications.


==> VLM_ALIGN_DRC_ARXIV/tex/5_conclusion.tex <==

%\vspace{-6pt}
%\section{Conclusion and Future Works}
% \vspace{-4pt}
%Local P\&R DRV fixing at advanced nodes is bottlenecked by two challenges: the scarcity of structured layout--violation training data and the domain gap between general-purpose VLMs and proprietary, topology-dependent design rules. We presented SCALE, a self-supervised framework that addresses both by generating diverse, signoff-verified multi-layer layout--violation pairs conditioned on real BEOL context and text-specified rule constraints, without requiring violation labels. The resulting domain-adapted DRC-VLM provides rule-aware geometric analysis that raises SOTA coding agents' average solve rate from 74.0\% to 92.5\% on 100 real sub-2\,nm fixing scenarios, demonstrating that self-supervised layout generation can bridge the gap between general-purpose VLMs and advanced-node DRC reasoning without rule-by-rule engineering.
%Future work will extend the dataset and VLM supervision to long-horizon, dynamic DRV fixing scenarios, where resolving one violation may cascade into new conflicts requiring multi-step repairs and iterative agent--checker feedback across larger layout regions.
%\textcolor{blue}{Future work will extend the dataset and VLM supervision to long-horizon, dynamic DRV fixing scenarios, where resolving one violation may cascade into new conflicts requiring multi-step repairs and iterative agent--checker feedback across larger layout regions, as well as to violations that demand net-level rerouting beyond the local repair scope.}

\vspace{-6pt}
\section{Conclusion and Future Works}
%Local P\&R DRV fixing at advanced nodes is bottlenecked by the scarcity of structured layout--violation training data and the domain gap between general-purpose VLMs and proprietary, topology-dependent design rules.
%We presented \emph{SCALE}, a self-supervised framework that addresses both by generating diverse, signoff-verified multi-layer layout--violation pairs conditioned on real BEOL context and text-specified rule constraints, without requiring violation labels.
%The resulting domain-adapted DRC-VLM provides rule-aware geometric analysis that boosts SOTA agents' solve rates by +12--25\% (up to 97\%) on 100 real sub-2\,nm cases, demonstrating that self-supervised layout generation can bridge general-purpose VLMs to advanced-node DRC reasoning without rule-by-rule engineering.
%By replacing manual template construction with scalable, data-driven domain adaptation, \emph{SCALE} offers a path toward automated design closure as rule complexity grows.
% Future work will extend to cascading multi-step DRV fixing and net-level rerouting beyond the local repair scope, as well as adapting the self-supervised generation--fine-tuning paradigm to other geometry-intensive EDA tasks where proprietary rules and data scarcity pose similar challenges.
Local P\&R DRV fixing at advanced nodes is bottlenecked by scarce layout--violation training data and the domain gap between general-purpose VLMs and proprietary design rules.
% We presented \emph{SCALE}, a self-supervised framework that addresses both by generating diverse, signoff-verified multi-layer layout--violation pairs conditioned on real BEOL context and text-specified rule constraints, without violation labels.
We presented \emph{SCALE}, a framework whose self-supervised generation stage produces diverse, DRC-annotated layout--violation pairs from real BEOL context without violation labels during training.
The domain-adapted DRC-VLM provides rule-aware geometric analysis that boosts SOTA agents' solve rates by +12--25\% (up to 97\%) on 100 real sub-2\,nm cases, demonstrating that scalable, data-driven domain adaptation can bridge general-purpose VLMs to advanced-node DRC reasoning without rule-by-rule engineering.
Future work will extend to cascading multi-step DRV fixing and net-level rerouting beyond the local repair scope, as well as adapting the self-supervised generation--fine-tuning paradigm to other geometry-intensive EDA tasks where proprietary rules and data scarcity pose similar challenges.




==> VLM_ALIGN_DRC_ARXIV/tex/_prefix.tex <==
% %\documentclass[conference]{acmart}
% %\documentclass[conference,9pt]{IEEEtran}
% % \documentclass[journal]{IEEEtran}
% \documentclass[sigconf,nobookmarks=true, 9pt]{acmart}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ACM related command
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setcopyright{none}
% \settopmatter{printacmref=false} % Removes citation information below abstract
% % \renewcommand\footnotetextcopyrightpermission{} % Removes footnote with conference information in the first column
% %\pagestyle{plain} % removes running headers
% \renewcommand\footnotetextcopyrightpermission[1]{} % removes footnote with conference information in first column
% % \copyrightyear{2023}
% % \acmYear{2023}
% \setcopyright{acmcopyright}\acmConference[\footnotesize{}]{}{}{} \acmBooktitle{28th Asia and South Pacific Design Automation Conference (ASP-DAC '23), January 16--19, 2023, Tokyo, Japan}
% \renewcommand\footnotetextcopyrightpermission[1]{}
%\pagestyle{plain}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{algorithm}
% \usepackage[noend]{algorithmic}
\usepackage{graphics}
\usepackage{booktabs}
\usepackage{graphicx}
\usepackage{subcaption}
\expandafter\def\csname ver@subfig.sty\endcsname{}
\usepackage{svg}
\usepackage{hyperref}
\usepackage{amsmath}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{lipsum}
\usepackage{enumitem}
\usepackage[super]{nth}
\usepackage[normalem]{ulem}

% \usepackage{algpseudocode}
% \usepackage[colorlinks=true]{hyperref}

\usepackage{algorithm}
\usepackage{algpseudocode}
\algtext*{EndWhile}
\algtext*{EndIf}
\algtext*{EndFor}
\algtext*{EndProcedure}

\usepackage{listings}
\lstdefinestyle{jsonsmall}{
  basicstyle=\ttfamily\scriptsize,
  breaklines=true,
  frame=single,
  rulecolor=\color{gray},
  backgroundcolor=\color{white},
  columns=fullflexible,
  keepspaces=true,
  aboveskip=2pt,
  belowskip=2pt,
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Space-Saving Settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Table rule thickness
\setlength{\heavyrulewidth}{0.08em}

% Caption
% \captionsetup[figure]{font=small}
\captionsetup{font=small}
\setlength{\abovecaptionskip}{1pt}
\setlength{\belowcaptionskip}{0pt}

% Float spacing
\setlength{\textfloatsep}{5pt plus 1.0pt minus 1.0pt}
\setlength{\floatsep}{4pt plus 1.0pt minus 1.0pt}
\setlength{\intextsep}{4pt plus 1.0pt minus 1.0pt}

% Layout margins
% \setlength{\textwidth}{7.5in} %7.4in
% \setlength{\linewidth}{7in} %7.4in
% \setlength{\columnsep}{1.0pc}
% \setlength{\topmargin}{-0.7in}
% \setlength{\headheight}{0.0in}
% \setlength{\oddsidemargin}{-0.45in}
% \setlength{\evensidemargin}{-0.45in}
% % \graphicspath{{./_fig/}}
% % \addtolength{\topmargin}{-.2in}
%\setlength{\textheight}{9.6in}
\setlength{\columnsep}{1pc}
\setlength{\topmargin}{-0.6in}
% acmart rejects manual \baselinestretch overrides.

% Section/subsection spacing (uncomment to tighten)
% \makeatletter
% \renewcommand{\section}{\@startsection{section}{1}{\z@}
%   {1.2ex plus 0.4ex minus 0.2ex}{0.6ex plus 0.1ex minus 0.1ex}
%   {\normalfont\large\bfseries\centering}}
% \renewcommand{\subsection}{\@startsection{subsection}{2}{\z@}
%   {0.8ex plus 0.3ex minus 0.2ex}{0.4ex plus 0.1ex minus 0.1ex}
%   {\normalfont\normalsize\bfseries}}
% \renewcommand{\paragraph}[1]{\@startsection{paragraph}{4}{\z@}
%   {0.4ex plus 0.1ex minus 0.1ex}{-1em}
%   {\normalfont\normalsize\itshape}{#1}}
% \makeatother

% Baseline stretch (uncomment to compress line spacing)
% \renewcommand{\baselinestretch}{0.98}

% List spacing (uncomment to tighten itemize/enumerate)
% \setlist{nosep, topsep=0pt, leftmargin=*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New Commands & Theorems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Colors
\definecolor{mygreen}{RGB}{79,173,91}
\newcommand{\imprv}[1]{\textcolor{blue}{#1}}
\newcommand{\gl}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\todo}[1]{\textcolor{red}{#1}}

% Pseudocode
\renewcommand{\algorithmicforall}{\textbf{for}}
\renewcommand\algorithmicthen{}
\renewcommand\algorithmicdo{}
\newcommand{\BREAK}{\STATE \textbf{break} }
\newcommand{\FOREACH}[1]{\FOR{\textbf{each} #1}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
% \renewcommand{\algorithmiccomment}[1]{// #1}

% Math
\newcommand{\sigmoid}{\mbox{$\mathit{Sigmoid}$}}
\newcommand{\threshold}{\mbox{$\mathit{threshold}$}}
\newcommand{\pred}{\mbox{$\mathit{pred}$}}
\newcommand{\adv}{\mbox{$\mathit{adv}$}}
\newcommand{\MSE}{\mbox{$\mathit{MSE}$}}

% Theorems
\newtheorem{problem}{Problem}
% \newtheorem*{problem*}{Problem}
\newtheorem{Definition}{Definition}
\newtheorem{Theorem}{Theorem}
\newtheorem{Proof}{Proof}
\newtheorem{Proposition}{Proposition}
\newtheorem{Lemma}{Lemma}
\def\code#1{\texttt{#1}}
% \IEEEoverridecommandlockouts

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Misc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\def\@mkbibcitation{\relax}
\makeatother

% \IEEEpubid{\makebox[\columnwidth]{978-1-6654-3274-0/21/\$31.00~\copyright2021~IEEE \hfill} \hspace{\columnsep}\makebox[\columnwidth]{ }}
% 978-1-6654-3274-0/21/$31.00 ©2021 IEEE
% \usepackage[utf8]{inputenc}

% Unicode character handling
\DeclareUnicodeCharacter{FF0C}{,}
\DeclareUnicodeCharacter{FF08}{(}
\DeclareUnicodeCharacter{FF09}{)}
\DeclareUnicodeCharacter{FF5E}{\textasciitilde} % Full-width tilde

% color definition


==> VLM_ALIGN_DRC_ARXIV/tex/timeline.tex <==
% \section{Collaborations}
% This project is in collaborations with multiple research and product team members including Walker Turner, Yoshi Nishi, Yan He, Yagaung Li, Nithin Kumar Mali, Ting Ku, Chen-chia Chang, Abhishek Akkurand, Georgios Kalogerakis, Sanquan Song, Frank Chang, Tsunghsun Hsieh, Chandrashekara Babu Rama, Chen Cui, Bobby Chen, Joosung Yoon and many others.


==> figtexs/DR_illustration.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/Figures_for_Complex_rules_illustration.pdf}    \caption{Illustration of VIA layer design rules. (1) \textbf{Basic Rules:} (R1-W) VIA widths are restricted to discrete allowed values $\{W_a, W_b, W_c, \ldots\}$; (R2-Sxx) minimum spacing thresholds are conditioned on the widths of both neighboring VIAs ($W_1$ and $W_2$). (2) \textbf{Group Rules and Group-Conditioned Spacing:} (R3-G) VIAs within a spacing range $[C_1, C_4]$ form groups (e.g., VIA\_GROUP\_2/3) with a maximum count $C_5$ per group; (R2.1-SxxGxH/V) spacing constraints within groups further depend on VIA width, group assignment, orientation (horizontal/vertical), and the parallel run length (PRL) region.}
    \Description{Diagram illustrating VIA design rules including width, spacing, grouping, and group-conditioned spacing constraints.}
    \label{fig:DR}
\end{figure}

==> figtexs/Dataset_Aug.tex <==
\begin{figure}[!t]
    % \vspace{-8pt}
    \centering
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/design.pdf}
        \caption{Human design.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/qwen_aug.pdf}
        \caption{Model augmented.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/script_gen.pdf}
        \caption{Script generated. }
    \end{subfigure}

    \caption{Comparison of layout generation methods. Layers are color-coded: \textbf{\textcolor{blue}{Blue} (Mx-1)}, \textbf{\textcolor{green}{Green} (Mx\_A)}, \textbf{\textcolor{cyan}{Cyan} (Mx\_B)}, and \textbf{\textcolor{red}{Red} (VIAx-1)}. (a) Original human-designed layout. (b) Model-augmented layout: the model preserves the original metal routing while generating different via patterns, creating realistic training diversity without altering the routing topology. (c) Script-generated layout: metals and vias are generated using rule-based scripts, resulting in unrealistic metal and via patterns that differ substantially from those found in real designs.}
    % \Description{Three layout crops comparing human-designed, model-augmented, and script-generated VIA placements on metal routing.}
    \label{fig:dataset_aug}
\end{figure}

==> figtexs/LayRep.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figs/LayRep_graph_v1.pdf}
%     \caption{Text-formulated layout representation. \textit{Top}: Each polygon is serialized as a coordinate-and-delta token sequence enclosed by \texttt{[Poly]}~\ldots~\texttt{[\textbackslash Poly]} delimiters and grouped under its layer header. \textit{Bottom}: In a real layout crop, metal polygons that extend beyond the crop boundary are marked with \texttt{[BPoly]} (Boundary Polygon) tokens, while fully interior polygons use \texttt{[Poly]}. The LLM receives conditional mixed \texttt{[BPoly]}/\texttt{[Poly]} from different layers as input and generates \texttt{[Poly]} as output, preventing edge-clipping artifacts and enclosure violations from boundary-clipped metal shapes.}
%     \Description{Diagram showing text serialization of layout polygons with coordinate-delta tokens and boundary polygon markers.}
%     \label{fig:layout_representation}
% \end{figure*}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/LayRep_graph_singlecolumn.pdf}
    \caption{Text-formulated layout representation. \textit{Top}: Each polygon is serialized as a coordinate-and-delta token sequence enclosed by \texttt{[Poly]}~\ldots~\texttt{[\textbackslash Poly]} delimiters and grouped under its layer header. \textit{Bottom}: In a real layout crop, metal polygons that extend beyond the crop boundary are marked with \texttt{[BPoly]} (Boundary Polygon) tokens, while fully interior polygons use \texttt{[Poly]}. The LLM receives conditional mixed \texttt{[BPoly]}/\texttt{[Poly]} from different layers as input and generates \texttt{[Poly]} as output, preventing edge-clipping artifacts and enclosure violations from boundary-clipped metal shapes.}
    \Description{Diagram showing text serialization of layout polygons with coordinate-delta tokens and boundary polygon markers.}
    \label{fig:layout_representation}
\end{figure}

==> tabtex/Ablation1_DataScaling.tex <==
% 50 samples version (archived)
% \begin{table}[!t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Training Samples} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} \\
% \midrule
% 2K            & 20.6\% $\pm$ 2.9\% & 31.7\% $\pm$ 5.3\% & 24.9\% $\pm$ 3.6\% & 6.3\% $\pm$ 1.3\% \\
% 5K            & 26.0\% $\pm$ 2.9\% & 36.9\% $\pm$ 5.7\% & 30.5\% $\pm$ 3.5\% & 8.4\% $\pm$ 1.8\% \\
% 8K            & 24.8\% $\pm$ 2.5\% & \textbf{38.4\%} $\pm$ 3.8\% & 30.2\% $\pm$ 2.7\% & 11.1\% $\pm$ 2.2\% \\
% 16K (full)    & \textbf{44.2\%} $\pm$ 3.5\% & 38.2\% $\pm$ 4.3\% & \textbf{41.0\%} $\pm$ 3.5\% & \textbf{18.3\%} $\pm$ 3.6\% \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Ablation: Effect of training data scale on Mixed (Ours) model (50 samples, $k$=10 trials, avg-trial metrics with 95\% bootstrap confidence intervals). Each model is trained for 1 epoch at GBS=8.}
% \label{tab:ablation_data_scaling}
% \end{table}


%100 samples version
\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Training Samples} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} \\
\midrule
2K            & 21.7\% $\pm$ 2.0\% & 33.7\% $\pm$ 3.5\% & 26.4\% $\pm$ 2.3\% & 7.1\% $\pm$ 1.1\% \\
5K            & 25.4\% $\pm$ 2.3\% & 37.9\% $\pm$ 3.6\% & 30.4\% $\pm$ 2.5\% & 9.0\% $\pm$ 1.7\% \\
10K           & 35.0\% $\pm$ 2.8\% & \textbf{52.5\%} $\pm$ 4.0\% & 42.0\% $\pm$ 3.1\% & 14.9\% $\pm$ 2.6\% \\
16K (full)    & \textbf{46.1\%} $\pm$ 2.8\% & 40.7\% $\pm$ 3.3\% & \textbf{43.3\%} $\pm$ 2.8\% & \textbf{20.7\%} $\pm$ 3.0\% \\
\bottomrule
\end{tabular}%
}
\caption{Ablation: Effect of training data scale on Mixed (Ours) model (100 samples, $k$=10 trials, avg-trial metrics with 95\% bootstrap confidence intervals). Each model is trained for 1 epoch at GBS=8.}
\label{tab:ablation_data_scaling}
\end{table}


==> tabtex/Ablation2_DataSource.tex <==
% 50 samples version (archived)
% \begin{table}[h]
% \centering
% \caption{Ablation: Effect of data augmentation source and reasoning traces (50 samples, 13 rules, $k$=10 trials). All models trained for 500 iterations. Training data compositions are detailed in Table~\ref{tab:data_composition}.}
% \label{tab:ablation_data_source}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model Variant} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} \\
% \midrule
% No-reason + ScriptGen aug. & 18.8\% & 37.3\% & 25.0\% &  6.3\% \\
% No-reason + ModelGen aug.  & 37.7\% & 37.9\% & 37.8\% & 17.9\% \\
% Reason + ModelGen aug.     & 44.2\% & 38.2\% & \textbf{41.0\%} & 18.3\% \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[h]
\centering
\caption{Ablation: Effect of data augmentation source and reasoning traces (100 samples, 13 rules, $k$=10 trials). All models trained for 500 iterations. Training data compositions are detailed in Table~\ref{tab:data_composition}.}
\label{tab:ablation_data_source}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Model Variant} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} \\
\midrule
No-reason + ScriptGen aug. & 19.9\% & 39.9\% & 26.6\% &  6.6\% \\
No-reason + ModelGen aug.  & 36.2\% & 36.9\% & 36.5\% & 16.7\% \\
Reason + ModelGen aug.     & \textbf{46.1\%} & 40.7\% & \textbf{43.3\%} & \textbf{20.7\%} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tabtex/DRUnderstanding.tex <==
\begin{table}[h]
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{\textbf{Soft (Rule)}} & \multicolumn{2}{c}{\textbf{Soft (Rule+Loc)}} & \multicolumn{2}{c}{\textbf{Hard (Rule)}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\textbf{Model} & \textbf{P@1} & \textbf{P@3} & \textbf{P@1} & \textbf{P@3} & \textbf{P@1} & \textbf{P@3} \\
\midrule
Qwen 3.5-397B  & 10.4\% & 25.2\% & 7.0\%  & 16.4\% & 0.8\% & 2.4\% \\
GPT-5.2        & 16.9\% & 29.5\% & 15.1\% & 26.1\% & 0.0\% & 0.0\% \\
Gemini 3 Pro   & 20.6\% & 29.0\% & 15.1\% & 22.4\% & 0.0\% & 0.0\% \\
Gemini 2.5 Pro & 27.7\% & 46.2\% & 15.3\% & 26.0\% & 2.8\% & 8.4\% \\
Nemotron-12B   & 33.3\% & 51.2\% & 14.1\% & 20.8\% & 2.4\% & 6.6\% \\
\bottomrule
\end{tabular}%
}
\caption{Model Performance Comparison across Soft and Hard Constraints}
\label{tab:model_performance}
\end{table}

==> tabtex/MainResults.tex <==
% 50 sample version (archived)
% \begin{table*}[t]
% \centering
% \caption{Model comparison on DRC VLM testing set (50 samples, 13 rules, $k$=10 trials, avg across trials). TP/FP/FN/TN are normalized rule-level rates (\%); overall metrics report 95\% bootstrap confidence intervals. Per-rule F1 columns report macro-average F1 (\%) within each rule category: \textbf{EN}~=~Enclosure (1 rule), \textbf{Grp}~=~Group (1 rule), \textbf{Spc}~=~Spacing (4 rules), \textbf{G-Spc}~=~Group-conditioned Spacing (4 rules), \textbf{W}~=~Width (1 rule). Training data compositions are detailed in Table~\ref{tab:data_composition}. \textsuperscript{$\dagger$}Ablation variants that isolate data source and reasoning contributions.}
% \label{tab:main_results}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lrrrr cccc | ccccc}
% \toprule
% & \multicolumn{4}{c}{\textbf{Confusion Matrix}} & \multicolumn{4}{c|}{\textbf{Overall Metrics}} & \multicolumn{5}{c}{\textbf{Per-Rule Category F1}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-14}
% \textbf{Model} & \textbf{TP}$\uparrow$ & \textbf{FP}$\downarrow$ & \textbf{FN}$\downarrow$ & \textbf{TN}$\uparrow$ & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} & \textbf{EN} & \textbf{Grp} & \textbf{Spc} & \textbf{G-Spc} & \textbf{W} \\
% \midrule
% \multicolumn{14}{l}{\textit{Commercial \& Open-Source Baselines}} \\
% % Qwen 3.5-397B     & 4.0\% & 2.1\% & 35.8\% & 58.1\% &  9.7\% $\pm$ 1.7\% & 20.1\% $\pm$ 3.8\% & 13.0\% $\pm$ 2.3\% &  2.5\% $\pm$ 0.9\% & -- & -- & -- & -- & -- \\
% GPT-5.2           & 6.7\% & 4.8\% & 33.2\% & 55.3\% & 15.4\% $\pm$ 3.6\% & 31.6\% $\pm$ 7.8\% & 20.7\% $\pm$ 4.8\% &  3.1\% $\pm$ 1.3\% &  0 & 41 & 35 &  5 &  0 \\
% Qwen3-VL-8B-Base  & 8.2\% & 6.0\% & 31.6\% & 54.1\% & 19.7\% $\pm$ 3.8\% & 29.7\% $\pm$ 6.0\% & 23.7\% $\pm$ 4.4\% &  2.4\% $\pm$ 1.1\% & 12 & 27 & 33 & 21 &  0 \\
% Gemini 3 Pro      & 8.2\% & 4.4\% & 31.6\% & 55.7\% & 19.9\% $\pm$ 2.7\% & \textbf{66.3}\% $\pm$ 9.1\% & 30.7\% $\pm$ 3.8\% &  8.4\% $\pm$ 2.2\% & \textbf{11} & \textbf{62} & 26 & 28 &  0 \\
% % Gemini 2.5 Pro    & 11.0\% & 10.0\% & 28.9\% & 50.1\% & 27.9\% $\pm$ 3.9\% & 37.7\% $\pm$ 5.6\% & 32.1\% $\pm$ 4.3\% & 11.0\% $\pm$ 2.6\% & -- & -- & -- & -- & -- \\
% % Nemotron-Nano-12B & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \midrule
% \multicolumn{14}{l}{\textit{Ours (Qwen3-VL-8B-SFT)}} \\
% \rowcolor{gray!8}
% \quad Mixed-NoR-ScriptGen\textsuperscript{$\dagger$} & 7.6\% & 2.4\% & 32.2\% & 57.8\% & 18.8\% $\pm$ 3.7\% & 37.3\% $\pm$ 7.9\% & 25.0\% $\pm$ 4.8\% &  6.3\% $\pm$ 2.1\% &  0 &  6 & 16 & 33 &  0 \\
% \rowcolor{gray!8}
% \quad Mixed-NoR-ModelGen\textsuperscript{$\dagger$}  & 14.6\% & 9.6\% & 25.2\% & 50.6\% & 37.7\% $\pm$ 4.6\% & 37.9\% $\pm$ 4.4\% & 37.8\% $\pm$ 3.9\% & 17.9\% $\pm$ 4.7\% &  0 & 29 & 30 & 52 &  5 \\
% \rowcolor{gray!15}
% \quad DRC-Reasoning-ModelGen\textsuperscript{$\dagger$} & 9.8\% & 4.6\% & 30.1\% & 55.5\% & 24.6\% $\pm$ 1.9\% & 61.5\% $\pm$ 5.2\% & 35.2\% $\pm$ 2.4\% & 12.3\% $\pm$ 2.0\% &  3 &  5 & 20 & 37 &  0 \\
% \rowcolor{gray!15}
% \quad Mixed (Ours)       & \textbf{17.4\%} & 14.2\% & \textbf{22.4\%} & 45.9\% & \textbf{44.2\%} $\pm$ 3.5\% & 38.2\% $\pm$ 4.3\% & \textbf{41.0\%} $\pm$ 3.5\% & \textbf{18.3\%} $\pm$ 3.6\% &  6 & 33 & \textbf{36} & \textbf{54} & \textbf{23} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


%100 sample version
\begin{table*}[t]
\centering
\caption{Model comparison on DRC VLM testing set (100 samples, 13 rules, $k$=10 trials, avg across trials). TP/FP/FN/TN are normalized rule-level rates (\%); overall metrics report 95\% bootstrap confidence intervals. Per-rule F1 columns report macro-average F1 (\%) within each rule category: \textbf{EN}~=~Enclosure, \textbf{Grp}~=~Group, \textbf{Spc}~=~Spacing, \textbf{G-Spc}~=~Group-conditioned Spacing, \textbf{W}~=~Width. Training data compositions are detailed in Table~\ref{tab:data_composition}. \textsuperscript{$\dagger$}Ablation variants that isolate data source and reasoning contributions.}
\label{tab:main_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrr cccc | ccccc}
\toprule
& \multicolumn{4}{c}{\textbf{Confusion Matrix}} & \multicolumn{4}{c|}{\textbf{Overall Metrics}} & \multicolumn{5}{c}{\textbf{Per-Rule Category F1}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-14}
\textbf{Model} & \textbf{TP}$\uparrow$ & \textbf{FP}$\downarrow$ & \textbf{FN}$\downarrow$ & \textbf{TN}$\uparrow$ & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{VIA Loc} & \textbf{EN} & \textbf{Grp} & \textbf{Spc} & \textbf{G-Spc} & \textbf{W} \\
\midrule
\multicolumn{14}{l}{\textit{Commercial \& Open-Source Baselines}} \\
Qwen3-VL-8B-Base  &  9.2\% &  6.1\% & 31.1\% & 53.7\% & 21.5\% $\pm$ 3.0\% & 31.1\% $\pm$ 4.6\% & 25.4\% $\pm$ 3.6\% &  3.7\% $\pm$ 1.1\% &  5\% & 23\% & 33\% & 26\% &  0\% \\
GPT-5.2           & 10.2\% &  6.7\% & 30.0\% & 53.1\% & 23.2\% $\pm$ 3.7\% & 45.7\% $\pm$ 7.8\% & 30.7\% $\pm$ 4.9\% &  4.2\% $\pm$ 1.3\% &  0\% & 48\% & 45\% &  9\% &  0\% \\
Gemini 3 Pro      & 10.7\% &  4.7\% & 29.5\% & 55.1\% & 25.8\% $\pm$ 2.7\% & \textbf{66.9\%} $\pm$ 6.2\% & 37.2\% $\pm$ 3.6\% & 11.0\% $\pm$ 1.7\% &  5\% & \textbf{75\%} & 34\% & 32\% &  0\% \\
\midrule
\multicolumn{14}{l}{\textit{Ours (Qwen3-VL-8B-SFT)}} \\
\rowcolor{gray!8}
\quad Mixed-NoR-ScriptGen\textsuperscript{$\dagger$} &  8.0\% &  2.3\% & 32.3\% & 57.4\% & 19.9\% $\pm$ 2.4\% & 39.9\% $\pm$ 4.9\% & 26.6\% $\pm$ 3.1\% &  6.6\% $\pm$ 1.5\% &  0\% &  7\% & 17\% & 34\% &  0\% \\
\rowcolor{gray!8}
\quad Mixed-NoR-ModelGen\textsuperscript{$\dagger$}  & 14.2\% &  8.9\% & 26.1\% & 50.8\% & 36.2\% $\pm$ 3.1\% & 36.9\% $\pm$ 3.5\% & 36.5\% $\pm$ 3.1\% & 16.7\% $\pm$ 3.2\% &  \textbf{8\%} & 27\% & 28\% & 51\% &  3\% \\
\rowcolor{gray!15}
\quad DRC-Reasoning-ModelGen\textsuperscript{$\dagger$} &  9.6\% &  4.8\% & 30.6\% & 54.9\% & 23.9\% $\pm$ 1.5\% & 59.2\% $\pm$ 3.7\% & 34.1\% $\pm$ 1.9\% & 11.1\% $\pm$ 1.7\% &  1\% &  5\% & 20\% & 36\% &  0\% \\
\rowcolor{gray!15}
\quad Mixed (Ours)       & \textbf{18.4\%} & 14.2\% & \textbf{21.8\%} & 45.6\% & \textbf{46.1\%} $\pm$ 2.8\% & 40.7\% $\pm$ 3.3\% & \textbf{43.3\%} $\pm$ 2.8\% & \textbf{20.7\%} $\pm$ 3.0\% &  2\% & 34\% & \textbf{37\%} & \textbf{57\%} & \textbf{14\%} \\
\bottomrule
\end{tabular}%
}
\end{table*}



==> tabtex/PerRuleF1.tex <==
\begin{table}[t]
\centering
\caption{Per-category average F1 (\%) across models (avg across $k$=10 trials, 50 samples). Column abbreviations: \textbf{GPT}~=~GPT-5.2, \textbf{Gem.}~=~Gemini~3~Pro, \textbf{Base}~=~Qwen3-VL-8B-Base, \textbf{S-NoR}~=~Mixed-NoR-ScriptGen\textsuperscript{$\dagger$}, \textbf{M-NoR}~=~Mixed-NoR-ModelGen\textsuperscript{$\dagger$}, \textbf{DRC}~=~DRC-Reasoning-ModelGen\textsuperscript{$\dagger$}, \textbf{Mixed}~=~Mixed (Ours). Daggers denote ablation variants.}
\label{tab:per_rule_f1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc|cccc}
\toprule
& \multicolumn{3}{c|}{\textbf{Baselines}} & \multicolumn{4}{c}{\textbf{Ours}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-8}
\textbf{Category} & \textbf{GPT} & \textbf{Gem.} & \textbf{Base} & \textbf{S-NoR\textsuperscript{$\dagger$}} & \textbf{M-NoR\textsuperscript{$\dagger$}} & \textbf{DRC\textsuperscript{$\dagger$}} & \textbf{Mixed} \\
\midrule
Enclosure (1)         &  0 & \textbf{11} & 12 &  0 &  0 &  3 &  6 \\
Group (1)             & 41 & \textbf{62} & 27 &  6 & 29 &  5 & 33 \\
Spacing (4)           & 35 & 26 & 33 & 16 & 30 & 20 & \textbf{36} \\
Group-cond.\ (4)      &  5 & 28 & 21 & 33 & 52 & 37 & \textbf{54} \\
Width (1)             &  0 &  0 &  0 &  0 &  5 &  0 & \textbf{23} \\
\midrule
\textbf{Macro-avg} (11) & 18 & 26 & 23 & 19 & 33 & 21 & \textbf{38} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tabtex/TokenCost.tex <==

\begin{table}[!t]
\centering
\caption{Token cost per local DRV fixing case. Average tokens are reported in thousands (K). Percentages under DRC-VLM-assisted values indicate token reduction relative to the corresponding baseline; negative values indicate increased token use.}
\label{tab:token_cost}
\scriptsize
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|rrrrrr}
\toprule
\multirow{2}{*}{\textbf{Method}}
& \multicolumn{6}{c}{\textbf{Avg. Tokens / Case (K)}} \\
\cline{2-7}
& EN & Width & Spacing & Color Spacing & Area & Overall
\\
\midrule
Claude Code
& 2{,}148.4
& 586.1
& 687.2
& 317.5
& 1{,}340.8
& 1{,}212.4 \\
\begin{tabular}[c]{@{}l@{}}DRC-VLM\\+ Claude Code\end{tabular}
& \begin{tabular}[c]{@{}r@{}}1{,}721.7\\{\scriptsize \textcolor{green!60!black}{(19.9\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}591.3\\{\scriptsize \textcolor{red}{(-0.9\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}665.8\\{\scriptsize \textcolor{green!60!black}{(3.1\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}172.7\\{\scriptsize \textcolor{green!60!black}{(45.6\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}1{,}330.4\\{\scriptsize \textcolor{green!60!black}{(0.8\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}1{,}028.1\\{\scriptsize \textcolor{green!60!black}{(15.2\%)}}\end{tabular} \\
\midrule
Codex
& 96.0
& 82.3
& 92.2
& 28.4
& 130.3
& 85.8 \\
\begin{tabular}[c]{@{}l@{}}DRC-VLM\\+ Codex\end{tabular}
& \begin{tabular}[c]{@{}r@{}}91.8\\{\scriptsize \textcolor{green!60!black}{(4.6\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}83.5\\{\scriptsize \textcolor{red}{(-1.4\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}88.9\\{\scriptsize \textcolor{green!60!black}{(3.6\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}29.8\\{\scriptsize \textcolor{red}{(-4.9\%)}}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}130.3\\{\scriptsize (0.0\%)}\end{tabular}
& \begin{tabular}[c]{@{}r@{}}83.9\\{\scriptsize \textcolor{green!60!black}{(2.2\%)}}\end{tabular} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex/timeline.tex <==
% \section{Collaborations}
% This project is in collaborations with multiple research and product team members including Walker Turner, Yoshi Nishi, Yan He, Yagaung Li, Nithin Kumar Mali, Ting Ku, Chen-chia Chang, Abhishek Akkurand, Georgios Kalogerakis, Sanquan Song, Frank Chang, Tsunghsun Hsieh, Chandrashekara Babu Rama, Chen Cui, Bobby Chen, Joosung Yoon and many others.

